WiForce: Wireless Sensing and Localization of Contact Forces on a Space Continuum

Contact force is a natural way for humans to interact with the physical world around us. However, most of our interactions with the digital world are largely based on a simple binary sense of touch (contact or no contact). Similarly, when interacting with robots to perform complex tasks, such as surgery, richer force information that includes both magnitude and contact location is important for task performance. To address these challenges, we present the design and fabrication of WiForce which is a 'wireless' sensor, sentient to contact force magnitude and location. WiForce achieves this by transducing force magnitude and location, to phase changes of an incident RF signal of a backscattering tag. The phase changes are thus modulated into the backscattered RF signal, which enables measurement of force magnitude and contact location by inferring the phases of the reflected RF signal. WiForce's sensor is designed to support wide-band frequencies all the way up to 3 GHz. We evaluate the force sensing wirelessly in different environments, including through phantom tissue, and achieve force accuracy of 0.3 N and contact location accuracy of 0.6 mm.

==> Makefile <==
TARGET           ?= main
TARGET_TYPE      ?= pdf
LATEXMK          ?= latexmk
LATEXDIFF        ?= latexdiff-vc

ifneq ($(V), 1)
Q                := @
LATEXMK_FLAGS    += -silent
else
Q                :=
LATEXDIFF_FLAGS  += -V
endif

UNAME_S          := $(shell uname -s)
TARGET_FILE       = $(TARGET).$(TARGET_TYPE)
TARGET_DIFF       = $(TARGET)-diff$(LATEXDIFF_BASE)

LATEXMK_FLAGS    += -$(TARGET_TYPE) -f

# Reference git branch/tag
LATEXDIFF_BASE   := submission2
LATEXDIFF_STYLE  := TRADITIONAL
# NOTE: vc-version does not take preamble
LATEXDIFF_FLAGS  += --git --flatten --force -r $(LATEXDIFF_BASE) 
LATEXDIFF_IGNORE := author,authornote,email,affiliation,institution,ccsdesc,renewcommand,section,subsecion,subsubsection
LATEXDIFF_NOENV  := (?:picture|DIFnomarkup|align|comment|CCSXML|thebibliography|figure|equation|tabular)[\w\d*@]*
LATEXDIFF_FLAGS  += --exclude-textcmd='$(LATEXDIFF_IGNORE)'

ifeq ($(shell which $(LATEXMK)), )
$(error "Please install `$(LATEXMK)`!")
endif
ifeq ($(shell which $(LATEXDIFF)), )
$(warning "Please install `latexdiff` or `latexdiff-vc` to use `make diff` function!")
endif

.PHONY: clean view check diff

$(TARGET_FILE): $(wildcard *.tex *.bib *.sty *.cls figures/*)
	@echo "Compiling..."
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET)

clean:
	@echo "Cleaning..."
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET) -C
	$(Q) rm -f $(TARGET).bbl $(TARGET_DIFF).bbl
	$(Q) if test -f $(TARGET_DIFF).tex; then $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET_DIFF) -C; rm $(TARGET_DIFF).tex; fi

view: $(TARGET_FILE)
ifeq ($(OS), Windows_NT)
	$(Q) open $(TARGET_FILE)
else
ifeq ($(UNAME_S), Linux)
	$(Q) xdg-open $(TARGET_FILE) &
endif
ifeq ($(UNAME_S), Darwin)
	$(Q) open $(TARGET_FILE) &
endif
endif

check: $(TARGET_FILE)
	$(Q) grep -i -e "undefined" -e "multiply" $(TARGET).log || echo "Nothing found."

# NOTE: latexdiff will not work with IEEEtran style
diff: clean
	@echo "Compiling diff..."
	$(Q) $(LATEXDIFF) $(LATEXDIFF_FLAGS) $(TARGET).tex
	$(Q) $(LATEXMK) $(LATEXMK_FLAGS) $(TARGET_DIFF)


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.


==> archive/intro-tkm.tex <==
% !TEX root = main.tex
% From a larger perspective where the problem stands and what people have tried
% one paragraph one message
% Dont put multiple messages 

\section{Introduction}

% 1.
% our sense of touch is important for our understanding of the world, yet in many applications we lose this sense of touch
% this often happens when we are interacting through a tool or some user interface --> give two examples
% to enable richer interactions and feedback of critical information, such as force, we need to improve our sensing capabilities
Our sense of touch is critical for understanding and interacting with the world around us. Human skin has \todo{four types of} mechanoreceptors capable of sensing force, vibration, texture, and slip, typically referred as haptic feedback\cite{abraira2013sensory}. When interacting with the physical world, we rely heavily on this haptic information for both input and feedback. However, due to a lack of force sensing capabilities in a number of emerging technologies, this critical haptic information is often lost. To enable richer interactions with digital world and/or feedback of task-critical force information like robotic surgery, there is a need to improve current force sensing capabilities.

% 2.
% Challenges with current sensing and what motivates the development of new sensors
% In smart surfaces/wearables/VR: space and power constraints
% In robotics/surgical robotics: space, particularly if you need multiple sensors

\begin{figure}[t]
  \centering
    % \placeholder[width=0.3\textwidth]{$l_1,l_2$ figure here}%
    \includegraphics[width=0.5\textwidth]{figures/introfig_v2_cropped.pdf}
  \caption{Applications targeted by \paperTitle: Surgical robots/tools inside the body inadvertently touch other tissues, leading to potential risks which can be avoided via haptic feedback. Finally, force sensitive robotic grippers could open up new automation possibilities.}
  \label{fig:appl}
\end{figure}

One area where this lack of sensing is particularly noticeable is in our interactions with the digital world, mostly via our smartphones, laptops and tablets. We are often limited to simple binary sense of touch, where contact force is either sensed or not sensed, and information about the magnitude of the force is generally lost. While this type of binary touch sensing is useful for controlling on/off type tasks, the lack of magnitude information makes control of analog tasks, including setting the volume or screen brightness, as non-intutive. Although, recently it has been demonstrate the multi-level force feedback~\cite{Apple3Dtouch,quinn2019estimating} when in contact with smartphones, to perform more than binary task, but still is limited. Imagine having the ability to sense force magnitude across a the tablet surface, it could significantly enhance the user experience. Further, the next generation of computing technologies, including smart surfaces, wearables, and augmented reality interfaces, could similarly benefit from such force sensing like a glove (shown in Fig.~\ref{fig:}). Ideally to enable all these applications, to harness force sensing, particularly for sensing across an entire surface, we need a mechanism to sense continuous force with the knowledge of the location of contact.



Another significant area, where the current lack of force sensing abilities poses a number of challenges, is robotics. Many robots are remotely teleoperated, typically due to the need to operate in environments that are either hazardous or physically difficult for humans to access. One challenge to force sensing in these scenarios is the development of sensors capable of operation in hazardous environments that can include, for example, extremely high temperatures or pressures. \todo{ref} Yet force sensing in these scenarios is critical, since teleoperation through a remote interface or tool causes the operator to lose their sense of touch, since they are no longer in direct contact with the physical environment. This lack of touch presents a particular challenge in the surgical setting, where robots can offer a number of potential benefits due to increased dexterity and precision compared to manual tools \cite{gomes2011surgical}. Without force feedback, surgeons can no longer ascertain whether or not the path taken by the robot or the amount of force applied to the tissue is safe \cite{alemzadeh2016adverse}. In addition, the sensing challenge is further exacerbated by the small size of surgical tools, as well as the need for force information not just at the tool tip, but ideally along the length of the tool as well. This exacerbates the need for force sensing from not only knowing the location and magnitude of force, but it should  be easy to attach, easy to read -- no wires, low-form factor and batteryless.  


% 3. 
% Propose to address these challenges through the development of a new sensor
Motivated by these requirements, we present \paperTitle, which makes a headway towards this direction with a new force sensor, capable of wirelessly sensing force magnitude and its location. The ability to sense forces wirelessly helps to address some of the difficulties inherent in sensing in remote environments (like in-body). It also helps to overcome issues of scaling when a large number of sensors are needed, since a large number of wires are no longer required. In addition, we have designed \paperTitle as a passive sensor by leveraging backscattering techniques. Rather than having an active RF transceiver with power amplifiers, ADC quantizers, and numerous other electronics, \name's force sensors have an antenna and a small identification unit and a force continuum surface, that directly embeds the force magnitude and location information in the properties of the signal reflected from the antenna. Such reflection requires minimal power, which can be harvested and therefore simplifies the sensor design. 

%Therefore, design consists of two main parts -- \paperTitle sensor and a wireless reader. Similar to traditional backscatter links, the wireless reader transmits a wireless signal, which is received and reflected back by the \paperTitle sensor, and the reader's receiving antenna receives %both the direct signal from the transmit antenna and 
%the reflected signal from the \paperTitle sensor. 

A natural question is how can force magnitude and location be embedded in the backscatterd signal. The key insight of \paperTitle sensor is to directly embed the applied forces and location to the changing the physical properties of reflected signals, instead of using an actual sensor to measure force and communicate wirelessly, saving electronics and power consumption. \name builds a novel surface, wherein it combines the classical beam mechanics and RF transmission line concepts to create the phase changes proportional to applied force and its location in the backscattered RF signals, without any additional electronics. \paperTitle consists of two parallel beams with a specialized polymer and a conductive trace on each and separated by air as shown in Fig.~\ref{}. As a the force is applied at a specific location, the top beam bends, causing the traces to connect. This phenomena can be viewed as a transmission line shorting and causing a reflection of signals. As the force increases, the locations of these shorting points changes on the both the end, causing a change in the phase of the reflected signal from both ends, which can be used to measure contact force and its location. \todo{check the both ends arguement}

If we can measure the absolute phase of the reflected signal from both the ends, we can enable accurate force magnitude and its contact location. Measuring aboslute phase on a wired measurement is quite trivial. However, when measuring the phase of the reflected signal it consists of wireless channel as well, furthermore many reflections of transmission signal from excitation radio, which impedes ability to measure the absolute phase. Instead, \paperTitle designs a novel architecture wherein a switch is added to both ends toggling at different frequency, connected by a single antenna instead one for each end. It builds novel algorithms to isolate the interference and measure the absolute phase by taking the length of sensor into account and making it a differential measurement.\todo{need to work on it again}

%WiForce consists of two parallel beams with a conductive trace on each and separated by air. From a mechanical viewpoint, when a force is applied to the top beam, the material bends, as dictated by beam mechanics models, and this bending causes the two traces to connect. From an RF viewpoint, this phenomena can be viewed as an air-substrate microstrip line. When the traces connect, they short-circuit this transmission line, reflecting the signals sent on both ends. As more force is applied, the surface bends further, which shifts the shorting points further towards the ends (Fig. \ref{fig:shorting_len}). The phases therefore travel a shorter length along the transmission line before getting reflected, allowing us to relate this change in phase to the magnitude and location of force applied.

In order to ensure accurate wireless sensing, we design a novel phase sensing algorithm which requires only periodic channel estimates and can thus work with any wideband channel sensing waveform. The algorithm views the switching of the signal at the sensor as an artificial-doppler, which allows it to isolate the signal from the environment in the doppler domain.
We designed and fabricated the sensor with \todo{with xx polymer and soft material} with bending properties which maximizes the phase, which was retrofitted with a RF-switches and a antenna. The power consumption of our sensor is $xx\mu$W evaluated in TSMC technology node of 65 nm, as flip chip package. The fabricated sensor works for the entire sub-3 GHz verified with the test equipment (vector network analyzer). We evaluated the \paperTitle sensor abilities to report force magnitude and location in multiple different settings in indoors, and inside body like environment using gelatin. We used USRP radios as the readers, and tested the sensor at 900~MHz and 2.4~GHz, which are the two most popular ISM bands. We show that the sensor can be read up to 10 meters of range over the air, and show the algorithm working even when the propagation through over the gelatin based muscle/fat/skin tissue layers composition similar to the human body to demonstrate the surgical applications. We evaluated the performance by using very accurate accuator to provide ground-truth force and contact location.  We achieved phase sensing with an accuracy of about $1^{o}$, giving us a force resolution of $0.3$~N, and location accuracy of $0.3$~mm.  Finally, we even evaluated our force sensor with a user pressing with his hand, and we achieved force resolution of $0.3$~N, and location accuracy of $0.3$~mm.
We believe this is the first step towards enabling numerous force sensing applications.

\begin{figure}[t!]

  \centering
  % include first image
  \includegraphics[width=0.5\textwidth]{figures/design_intro.pdf}
  \caption{As contact force increases, the top beam bends and shifts the shorting points (dotted lines). Reflected signal phase changes as the shorting points shifts. Hence sensing phases from the either ends ($\phi_1,\phi_2$) allows force estimation}
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=\linewidth]{figures/phase_to_len.pdf} 
%   \caption{Reflected signal phase changes depend on length travelled on the transmission line until being reflected from the shorting point. Hence sensing these phases from the either ends ($\phi_1,\phi_2$) allows us to locate the shorting points and hence allows to estimate force magnitude.}
%   \label{fig:phase_v_len}
% \end{subfigure}
\label{fig:intro_fig}
\end{figure}




% The key enabling technology to achieve this seamless wirelees sensing was to leverage `backscatter sensing', in which instead of having an active RF toolchain with power amplifiers, ADC quantizers and bunch of other electronics, these sensors just had an antenna and a small identification chip, which directly embedded the touch information in the properties of the signal reflected off from the antenna. Hence, the major question answered by \paperTitle is, how can we backscatter force information, rather than just touch. Such  

% % Not sure if we need this here
% \paperTitle's sensor consists of two parts, the force to phase transduction mechanism and ensuring robust interference-free wireless connectivity. The wireless connectivity ensures that this phase information is embedded in a high speed wireless channel, enabling low-power wireless force feedback. Said differently, instead of generating wireless signals, \paperTitle conveys the force information in the channel of the interference-free reflected signals. Furthermore, \paperTitle is wideband and works at all frequencies up to 3 GHz, allowing the reader to be WiFi, Radar or even RFID. 

% Hence, doing so, it is not required to generate and transmit wireless signals at the sensor, since all the force information is directly encoded into the phase of the reflected signal, which makes the solution low-powered.
% Such a wireless force sensor can enable safe, battery-free operation of force sensing surgical robots inside the body and can enable the creation of passive force sensitive surfaces. The two broad themes which \paperTitle's sensor design targets are providing haptic feedback for surgical robots, and smart force sensitive passive surface designs which could be used for HCI.


% Explaining on high level the transduction mech'm
% This increased contact length around the initial contact location between the beams changes the signal phase from both the ends, hence relating the applied contact force $F$ with the phase changes from either ends of the sensor.

% I think most of these ideas have been told before, we can explictly call out Bluettoth etc 
% The next challenge lies in, how to communicate this shorting point location wirelessly. One way to estimate this could be to generate a RF signal and use it to measure the length at which this short-circuit arises, and then sample/quantize the information and communicate wirelessly using a radio technology like Bluetooth. However, the above overall process would consume significant power and energy, and would make the sensor bulky. In contrast, \paperTitle combines the communication and sensing of the force into a single paradigm. Our key idea is to equip both sides of the sensor with an antenna which can reflect the signal after traveling some length on the transmission line before encountering the short circuit and reflecting back, in effect encoding the contact information onto reflected phases. Such reflection requires no power, and simplifies the sensor design. Furthermore, we can use any external radio to send a signal, and the reflected signal when measured by external radio could estimate the length/additional phase traveled before the short circuit.

% and then how to do it accurately
%A natural next challenge is to measure very accurately the reflection properties arising from \paperTitle's sensor, so that the wireless reader can estimate the phase changes accurately. Typically, when an external radio sends signals out in the environment, it receives many reflections back. In this sea of reflections, \paperTitle needs to identify the reflection corresponding to the sensor and measure its phases. To separate the reflection signal from the rest of the reflections, we add a switch, which toggles at a certain frequency, between the antenna and the sensor. The frequency of switching gives the sensor a unique signature and thus enables us to identify the sensor and isolate the reflection's properties. We do so by uniquely corresponding to the sensor via its signature and the wireless reader design can read multiple sensors by choosing different toggling frequencies. 

% Summarizing the contributions
%In summary, \paperTitle builds a backscatter tag which causes phase shifts in the reflected signal depending on the force applied. Then, we measure the phase shift on the external receiver to infer the force. \paperTitle forms analog modulation with backscatter communication and enables measurement of the force.A natural question is how to decode the analog phase information from the sensor. For this, \paperTitle designs a novel phase sensing algorithm which just requires periodic channel estimates and can thus work with any wideband channel sensing waveform.\paperTitle's algorithm views the switching of the signal at the sensor as an artificial-doppler, which allows it to isolate the signal from the environment in doppler domain.After this separation, \paperTitle's phase sensing algorithm allows us to measure the phase changes from the sensor over the entire bandwidth of the signal, which facilitates phase sensing with an accuracy of about $1^{o}$. This gives us a force resolution of $0.3$~N, with ultra high contact location accuracy of $0.3$~mm. We prototype \paperTitle using a sensor consisting of a soft beam attatched to the top of the microstrip line, which, when pressed, shorts the ground trace at different positions on the fixed beam below.
%which provide low loss and consumes low power, which is driven by a ring-oscillator implemented on the FPGA. 


% \todo{agrim I have commented the part below, please feel free to bring it back... }


%A key question which \paperTitle answers is, how can contact force, which is a purely mechanical parameter, be linked to RF signal phase. \paperTitle does this by combining RF and mechanical viewpoint of a simple beam model, consisting of two parallel traces, one being ground trace and other being the signal trace, separated by air. 


%In RF viewpoint, this is basically a microstrip transmission line with air as substrate, whereas in a mechanical viewpoint this is basically a cantilever beam model. Viewing the sensor as a cantilever beam model allows mapping forces to contact lengths $l_1$, $l_2$ (Fig. \ref{fig:intro_fig}). Viewing the sensor as a microstrip transmission line allows us to map reflected signal phases to the contact locations where the transmission line gets shorted from either ends ($l_1, l_2$, Fig. \ref{fig:intro_fig}). Hence, by forming this connection between RF and mechanical viewpoints, \paperTitle is able to estimate contact force by observing the phase changes due to shorting of transmission line at different locations. 

%Further, \paperTitle designs a novel algorithm to detect this phase change accurate to about a degree, which leads to a force resolution of about 0.2 N. The algorithm takes inspiration from how FMCW/UWB systems estimate signal doppler variations, and uses this idea to give an artificial doppler to the sensor by making it switch at certain frequencies. The artificial doppler generated is high enough to make it isolated from any low doppler environmental signals. 
%This allows \paperTitle to estimate phase changes super accurately and robust even to dynamic multipath interference, and then map it back to contact force using the cantilever beam model.
%However, instead of testing the algorithm with specialized waveforms and ultra-high bandwidths, we show the algorithm working for OFDM based channel estimation to motivate seamless fusion of communication and sensing for this sensing paradigm.


% \paperTitle hence   in force sensing for surgical robots. The sensor can, in principle, sense as well as locate contact force across the robot body. This is achieved by abstracting the sensor as a transmission line model. A transmission line model is generated by viewing the sensor as a lumped model of continuous impedences, to provide data in a continuum fashion. The signal trace of the transmission line can be wrapped across the robotic manipulator, and ground layer being the inner diameter of the robot.This, in-effect act like an artificial skin for the robot. However, given the size limitations and the flexibility requirements, it is imperative that this sensor should provide wireless reading capabilities. 

% We leverage 2 key insights here, which allows us to create such an artificial skin capable of sensing force across the length. Firstly, by using mechanical models like cantilever beams etc, the force measure can be inferred by estimating the contact length of the flexible outer layer of skin, which has the signal trace of the transmission line, with the robotic surface acting as a ground layer. To estimate this contact length, we measure the contact lengths from the either end of the transmission line. This is done by measuring the phase change in the signal due to this pressing motion, as the signal now travels a lesser length before reflecting back. The second key insight we have here is that, since all the force information is encoded in the phase change of the signal, this sensing modality can be readily integrated with wireless sensing paradigms, which also leverage sensor data information encoded in phase of the signal. To do so, we have antennas on either ends of the transmission line, and we perform wireless measurements of phase change induced onto either end of the transmission line, in order to estimate the force location and force magnitude. For this, we address issues like intermodulation harmonics, clock drift and multipath correction, to estimate the phase changes accurately and precisely.

% Hence the technical contributions of this paper are
% \begin{itemize}
%   \item Ideation and fabrication of a novel force sensing paradigm involving transmission lines 
%   \item The sensor design is the first one to sense force position and location across the length of the robot
%   \item Performing double sided phase measurements from 2 antennas, and a novel algorithm to address the intermodulated harmonics
%   \item Performing accurate sensing of phase by eliminating clock drifts and cancelling multipath
% \end{itemize}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/sensor.pdf}
% \caption{Transmission line (yellow) is wrapped around the robot body and acts like an artificial skin layer. The contact force manifests as phase changes $\phi_1$,$\phi_2$ as the transmission line which was previously open ended is now shorted at two contact points}
% \end{figure}


==> archive/intro_acrosslength.tex <==
% !TEX root = main.tex

\section{Introduction}


Robotic manipulators have been very successful in automating tasks traditionally performed by human hands, in areas of application like industrial factories, exploration robotics and prosthetics. Furthermore, robotic manipulators hold a huge potential in surgery robotics, where they can go beyond mimicking a human hand and perform far more intricate surgeries than possible by a human hand. However, to achieve this, the current robots need to be sufficiently upgraded in terms of sensor modalities. 

Human skin is an extremely sensitive layer, you can feel the magnitude and contact location of even a slightest of nudge. Robotic manipulators on the other hand have no such sensitive layer, which prohibit them to sense magnitude and location of a contact force which they experience. This severely limits the application capabilities of these robots, to an extent that one of the main roadblock to enabling these precise robotic surgeries is that doctors can't ascertain if the path taken by the robot is safe or not \cite{alemzadeh2016adverse}. That is, doctors do not know, whether the robot is in contact with some organs/tissues or not, and whether the contact force is appreciable large to hurt the tissue. Hence, there has to be a feedback in terms of contact force sensing to help the doctors in identifying safe operation of the robot.

Force sensing for such medical robots has thus garnered a lot of research interest \cite{tegin2005tactile,trejos2010force}, however it still remains an unsolved problem. Force sensing has even been posed as a `Grand Challenge' in \cite{burgner2015continuum}. Typically force sensing has been attempted with sensing principles like strain gauges, load cells, FBG based optical fibres and force sleeves. Each of these sensing principles sense force only at a particular point, and not across the length. Worse, not one of these sensing principles is universally optimal. Depending on whether you would want to sense force at the tip, or near the robot-tissue interface, the appropriate choices are strain gauges and force sleeves respectively. Hence, there is a need for a sensing principle which can sense force across the length, and the main goal here should be that the sensing principle should, in effect provide a continuum artificial skin to the robot, instead of providing force measurement at discrete points.

The sensor developed by us tries to address this lacuna in force sensing for surgical robots. The sensor can, in principle, sense as well as locate contact force across the robot body. This is achieved by abstracting the sensor as a transmission line model. A transmission line model is generated by viewing the sensor as a lumped model of continuous impedences, to provide data in a continuum fashion. The signal trace of the transmission line can be wrapped across the robotic manipulator, and ground layer being the inner diameter of the robot.This, in-effect act like an artificial skin for the robot. However, given the size limitations and the flexibility requirements, it is imperative that this sensor should provide wireless reading capabilities. 

We leverage 2 key insights here, which allows us to create such an artificial skin capable of sensing force across the length. Firstly, by using mechanical models like cantilever beams etc, the force measure can be inferred by estimating the contact length of the flexible outer layer of skin, which has the signal trace of the transmission line, with the robotic surface acting as a ground layer. To estimate this contact length, we measure the contact lengths from the either end of the transmission line. This is done by measuring the phase change in the signal due to this pressing motion, as the signal now travels a lesser length before reflecting back. The second key insight we have here is that, since all the force information is encoded in the phase change of the signal, this sensing modality can be readily integrated with wireless sensing paradigms, which also leverage sensor data information encoded in phase of the signal. To do so, we have antennas on either ends of the transmission line, and we perform wireless measurements of phase change induced onto either end of the transmission line, in order to estimate the force location and force magnitude. For this, we address issues like intermodulation harmonics, clock drift and multipath correction, to estimate the phase changes accurately and precisely.

Hence the technical contributions of this paper are
\begin{itemize}
  \item Ideation and fabrication of a novel force sensing paradigm involving transmission lines 
  \item The sensor design is the first one to sense force position and location across the length of the robot
  \item Performing double sided phase measurements from 2 antennas, and a novel algorithm to address the intermodulated harmonics
  \item Performing accurate sensing of phase by eliminating clock drifts and cancelling multipath
\end{itemize}

\begin{figure}[H]
\centering
\includegraphics[width=0.5\textwidth]{figures/sensor.pdf}
\caption{Transmission line (yellow) is wrapped around the robot body and acts like an artificial skin layer. The contact force manifests as phase changes $\phi_1$,$\phi_2$ as the transmission line which was previously open ended is now shorted at two contact points}
\end{figure}


==> archive/intro_surface.tex <==
% !TEX root = main.tex
% From a larger perspective where the problem stands and what people have tried
% one paragraph one message
% Dont put multiple messages 

\section{Introduction}

% Contact force is fundamental
Contact force is a fundamental sensing measure that affects how we interact with the world around us.
Humans sense contact force via mechanoreceptors in our skin, which allows us to sense the magnitude and contact location of even the smallest forces \cite{abraira2013sensory}. 
However, in most of our interactions with the digital world, mostly via our smartphones, laptops and tablets, this rich force information is replaced with a simple sense of touch (contact or no contact). 
In other words, we mostly interact with these entities using only a binary sense of whether or not contact has occurred, while the information about the magnitude of the applied contact force is generally lost.

% Motivating force sensing on a high level
% In the next generation of user-interactions with upcoming technologies like smart surfaces, wearables and VR interfaces, interactions with different objects will necessitate sensing of full contact force information in addition to simple touch. 
% Apple and Google have already started exploring force feedback for richer UI experiences \cite{quinn2019estimating}, and the latest iPhones and Apple watches come equipped with capacitive force sensor \cite{Apple3Dtouch} to provide haptic feedback to the user. 
% Instead of providing the ability for continuum force sensing, which can enable intuitive UIs to control analog variables like volume/brightness, these sensors just provide an alternative to the traditional press and hold interfaces to perform binary tasks. 
% To harness the full potential of force controlled interfaces, it is required to sense continuum force instead of sensing digitized levels.  

% What force sensing will truly enable analog control, space constraint and power constraint (Vision should be there!)
Although contact sensing leads to intuitive control of binary tasks like play/pause, on/off and others, by itself, it fails to control more analog tasks like setting volume to a certain level, increasing screen brightness and others. Typically, these tasks are then supplemented by touching/swiping across the screen length to perform a gesture to control these analog tasks. In the next generation of user-interactions with upcoming technologies like smart surfaces, wearables and VR interfaces, almost all of which are form-factor and power constrained, having these analog gestures will not be possible, since there will be no space to perform these swiping gestures. As an example, Here lies the true potential of force sensing modalities, since these can provide control of these analog tasks using just one contact force sensor. Apple and Google have already started exploring force feedback for richer UI experiences \cite{quinn2019estimating}, and the latest iPhones and Apple watches come equipped with capacitive force sensor \cite{Apple3Dtouch} to provide haptic feedback to the user.

% Coming to Robotics now, which demands continuum sensing
Another significant area, where the current lack of force sensing abilities poses a number of challenges, is robotics. In particular, surgical robots offer a number of potential benefits due to increased dexterity and precision compared to manual procedures \cite{gomes2011surgical}. However, because many of these robots are teleoperated through a remote interface, rather than directly operated, surgeons lose their sense of touch. 
This lack of force feedback can make it challenging to ascertain whether or not the path taken by the robot or the amount of force applied to the tissue is safe \cite{alemzadeh2016adverse}. 
Force sensing has even been posed as a `Grand Challenge' for further advancement of surgical robotics \cite{burgner2015continuum}. 
The force sensing problem further exacerbates for robotics applications, since here haptic feedback is required not only at certain sensor mounting points, but over the entire length of the robot, and in effect act like a force sensitive skin for the robot.
Hence, there has to be continuum feedback in terms of contact force, as well as contact location sensing to help the doctors in identifying safe operations of the robot.
% \todo{what about moving second applicaiton area (medical) here instead? talk about the need... then move onto the part about continuum and wireless sensing?} Another significant area where the current lack of continuum force sensing abilities poses a number of challenges, is robotics, and in particular, surgical robotics. ......

\begin{figure}[t]
  \centering
    % \placeholder[width=0.3\textwidth]{$l_1,l_2$ figure here}%
    \includegraphics[width=0.5\textwidth]{figures/introfig_v2_cropped.pdf}
  \caption{Applications targeted by \paperTitle: Surgical robots/tools inside the body inadvertently touch other tissues, leading to potential risks which can be avoided via haptic feedback. Finally, force sensitive robotic grippers could open up new automation possibilities.}
  \label{fig:appl}
\end{figure}

% Set up wireless sensing bit, continuum problem has been set up
% One wires, sensor array would require wire
% Why would one wire make a big deal?
Working with space constraints naturally motivates the need of these sensing modalities to be able to sense wirelessly. 
That is, running wires around the robot to get force feedback, or having densely wired sensor-array to sense force across the surface violate these space constraint applications.
In addition, the problem is only made worse since these applications demand low-power solutions. 
In case of surgical robots, force sensing solutions requiring a bunch of electronics and higher power consumption pose coupled risks of harmful chemical leakage and capacitative discharges, both which can in turn harm the human tissues.
However, this low-power requirement goes against the wireless sensing requirements, since it would require substantial power to first encode sensor readings into bits, and then generate and transmit wireless signals to communicate the sensor readings wirelessly.
This essentially becomes a chicken and egg problem, where requiring wireless reading capabilities to satisfy space constraints give birth to power constraints since these wireless solutions would either require a battery, or a wired power connection, which would then go back and violate the space constraints.
Low-powered wireless force sensing solutions, that instead of requiring a battery, can meet the power requirements with harvested power from the surroundings, would be the panacea which breaks this chicken-and-egg loop for haptic feedback modalities.
Hence, this is the main design aim of \paperTitle is to create such a force sensor which can perform wireless force feedback with lowest power requirement possible.
 % Can go to related works
% To address the need of continuum sensing, recent work has utilized sensor arrays of small point sensors to create a macroscopic force sensitive surface\todo{refs}. 
% These point sensors can sense forces very accurately, however only do so over a very small force sensitive area, which fails to provide a space continuum.
% In order to achieve the required continuum granularity, a large number of these point sensors per unit area are required, which increases the reading latency and power consumption quadratically. 
% Given these limitations, these sensing surfaces can not accommodate seamless wireless capability, that is, to communicate the force sensing data over the air they need dedicated micro-controllers, a battery to meet the power requirements and form factor inaccurate RF transceivers.
% The sheer amount of electronics required for these solutions is antithesis to the requirements posed by these applications, where doctor might not want to risk electrical discharges to the tissue and harmful chemical leakage from the battery.
% To support seamless wireless sensing capability, these sensors need to have the form factor of a smart surface akin to just a small painting which can be hung around, or in form of small stickers which can be stuck in hard to mount places. 
% The binary touch based wireless sensing modalities have recently achieved both these goals, with leading research showing touch based sensing ranging from ubiquitous networked smart surfaces \cite{gao2018livetag} to small stickable RFIDs \cite{pradhan2017rio,li2016paperid}.
% However, none of these past works could sense beyond just contact/no contact and were totally oblivious to the magnitude of contact force the touch interaction happened with.
% The key enabling technology to achieve this seamless wirelees sensing was to leverage `backscatter sensing', in which instead of having an active RF toolchain with power amplifiers, ADC quantizers and bunch of other electronics, these sensors just had an antenna and a small identification chip, which directly embedded the touch information in the properties of the signal reflected off from the antenna. Hence, the major question answered by \paperTitle is, how can we backscatter force information, rather than just touch. Such  
% Worse, not one of these sensing principles is universally optimal. Depending on whether you would want to sense force at the tip, or near the robot-tissue interface, the appropriate choices are strain gauges and force sleeves respectively. 
% Robotic manipulators hold a huge potential in surgery robotics, where they can go beyond mimicking a human hand and perform far more intricate surgeries than possible by a human hand. However, unlike a human hand, these robotic manipulators are completely oblivious to the magnitude of force they touch their environment with.  Hence, there has to be a feedback in terms of continuum contact force sensing to help the doctors in identifying safe operation of the surgical robot inside the human body.
% Sensing touch interactions on surfaces has also attracted a lot of research interest in the wireless sensing community \cite{pradhan2017rio,li2016paperid,gao2018livetag}. The systems have demonstrated detection of gestures/swipes alongside simple touch events on passive surfaces, which have a lot of HCI applications of extending UIs to such passive surfaces. However, these works are limited in the sense that these can't distinguish events wherein a person is touching with higher/lower force, and in a way provide just 1 bit information related to the touch event.

% What does \paperTitle do, results and implementation in short
% Adding one line about what backscatter is on high level for people who might
% not know what it means. Also need to tell our paper is the first one to do so
\paperTitle presents the design, implementation and evaluation of a sensor prototype which can sense force, as well as it's application location, accurately and continuously throughout the sensor surface and thus addresses the low-power continuum sensing lacuna with the current force sensors. 
\paperTitle's design consists of two parts, backscatter enabled sensor and wireless reader. 
Similar to traditional backscatter links, the wireless reader transmits a wireless signal, which is received and reflected back by the backscatter tag, and the reader's receiving antenna receives both the direct signal from the transmit antenna and the reflected signal from the sensor.
The key idea of \paperTitle is to make the sensor transduce contact force into phase changes in these backscaterred RF signals, which are then estimated with the precision of $1^{o}$ by the wireless reader. 
This precision of phase sensing translates to a force magnitude sensing accuracy of about $0.3$~N, combined with an ultra accurate contact location sensing accuracy of $0.6$~mm.
Since the force magnitude is directly transduced onto the reflected signal phase, instead of going through the traditional quantize-encode-transmit strategy for wireless feedback, \paperTitle's solution meets the low-power requirements posed before, and is the first work which attempts to do so as well.

% % Not sure if we need this here
% \paperTitle's sensor consists of two parts, the force to phase transduction mechanism and ensuring robust interference-free wireless connectivity. The wireless connectivity ensures that this phase information is embedded in a high speed wireless channel, enabling low-power wireless force feedback. Said differently, instead of generating wireless signals, \paperTitle conveys the force information in the channel of the interference-free reflected signals. Furthermore, \paperTitle is wideband and works at all frequencies up to 3 GHz, allowing the reader to be WiFi, Radar or even RFID. 

% Hence, doing so, it is not required to generate and transmit wireless signals at the sensor, since all the force information is directly encoded into the phase of the reflected signal, which makes the solution low-powered.
% Such a wireless force sensor can enable safe, battery-free operation of force sensing surgical robots inside the body and can enable the creation of passive force sensitive surfaces. The two broad themes which \paperTitle's sensor design targets are providing haptic feedback for surgical robots, and smart force sensitive passive surface designs which could be used for HCI.

\begin{figure}[h]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/design_intro.pdf}
  \caption{As contact force increases, the top beam bends more and more, which shifts the shorting points towards the ends. Hence, the force magnitude can be sensed by locating the shorting points on the sensor. Past work with RFID based touch sensing could only sense contact/no contact}
  \label{fig:shorting_len}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/phase_to_len.pdf} 
  \caption{Reflected signal phase changes depend on length travelled on the transmission line until being reflected from the shorting point. Hence sensing these phases from the either ends ($\phi_1,\phi_2$) allows us to locate the shorting points and hence allows to estimate force magnitude}
  \label{fig:phase_v_len}
\end{subfigure}
\caption{Force to phase transduction mechanism.}
\label{fig:intro_fig}
\end{figure}

% Explaining on high level the transduction mech'm
A natural question arises as to how can contact force, a mechanical entity, be related to reflected signal phase, which is a RF signal parameter.
To make this connection, \paperTitle fabricates a sensor which consists of 2 parallel beams separated by a small air gap. 
To relate force and signal phase, this parallel beam sensor can be viewed from two classical viewpoints -- mechanical and RF domains.
From a mechanical viewpoint, the bending of the sensor in the presence of a contact force is dictated by popular beam bending mechanical models.
From a RF viewpoint, these two parallel beams separated by air act like an air-substrate microstrip line, which allows us to relate signal phase with the length traveled by the signal on the transmission lines.
A confluence of these viewpoints allows \paperTitle to relate mechanical contact force with RF signal phases (Fig. \ref{fig:intro_fig}).
When a force is applied to the top of the beam, the material bends and connects with the rigid fixed beam that contains a ground trace, short-circuiting the transmission line and reflecting the signals sent on both ends. 
% The unique mapping between force application location and measured phase change at both ends of the trace allows to create a relationship between these entities. 
As one applies more force, the surface bends further, which shifts the shorting points further towards the ends (Fig. \ref{fig:shorting_len}). 
Due to the shifting of shorting points as force magnitude increases, the phases travel lesser length on the transmission line before getting reflected, which allows \paperTitle to relate this change in phase to the magnitude of force applied.
% This increased contact length around the initial contact location between the beams changes the signal phase from both the ends, hence relating the applied contact force $F$ with the phase changes from either ends of the sensor.

% I think most of these ideas have been told before, we can explictly call out Bluettoth etc 
% The next challenge lies in, how to communicate this shorting point location wirelessly. One way to estimate this could be to generate a RF signal and use it to measure the length at which this short-circuit arises, and then sample/quantize the information and communicate wirelessly using a radio technology like Bluetooth. However, the above overall process would consume significant power and energy, and would make the sensor bulky. In contrast, \paperTitle combines the communication and sensing of the force into a single paradigm. Our key idea is to equip both sides of the sensor with an antenna which can reflect the signal after traveling some length on the transmission line before encountering the short circuit and reflecting back, in effect encoding the contact information onto reflected phases. Such reflection requires no power, and simplifies the sensor design. Furthermore, we can use any external radio to send a signal, and the reflected signal when measured by external radio could estimate the length/additional phase traveled before the short circuit.

% and then how to do it accurately
A natural next challenge is to measure very accurately the reflection properties arising from \paperTitle's sensor, so that the wireless reader can estimate the phase changes accurately. Typically, when an external radio sends signals out in the environment, it receives many reflections back. In this sea of reflections, \paperTitle needs to identify the reflection corresponding to the sensor and measure its phases. To separate the reflection signal from the rest of the reflections, we add a switch, which toggles at a certain frequency, between the antenna and the sensor. The frequency of switching gives the sensor a unique signature and thus enables us to identify the sensor and isolate the reflection's properties. We do so by uniquely corresponding to the sensor via its signature and the wireless reader design can read multiple sensors by choosing different toggling frequencies. 

% Summarizing the contributions
In summary, \paperTitle builds a backscatter tag which causes phase shifts in the reflected signal depending on the force applied. 
Then, we measure the phase shift on the external receiver to infer the force. 
\paperTitle forms analog modulation with backscatter communication and enables measurement of the force.
A natural question is how to decode the analog phase information from the sensor. 
For this, \paperTitle designs a novel phase sensing algorithm which just requires periodic channel estimates and can thus work with any wideband channel sensing waveform.
\paperTitle's algorithm views the switching of the signal at the sensor as an artificial-doppler, which allows it to isolate the signal from the environment in doppler domain.
After this separation, \paperTitle's phase sensing algorithm allows us to measure the phase changes from the sensor over the entire bandwidth of the signal, which facilitates phase sensing with an accuracy of about $1^{o}$. This gives us a force resolution of $0.3$~N, with ultra high contact location accuracy of $0.3$~mm. We prototype \paperTitle using a sensor consisting of a soft beam attatched to the top of the microstrip line, which, when pressed, shorts the ground trace at different positions on the fixed beam below.
%which provide low loss and consumes low power, which is driven by a ring-oscillator implemented on the FPGA. 
The fabricated sensor works for entire sub-3 GHz verified with the vector network analyzer. We used USRP radios as the readers, and tested the sensor at 900~MHz and 2.4~GHz, two most popular ISM bands. We show that the sensor can be read up to 10 meters of range over the air, and show the algorithm working even when the propagation through over the gelatin based muscle/fat/skin tissue layers composition similar to the human body to motivate the surgical applications.

% \todo{agrim I have commented the part below, please feel free to bring it back... }

\if 0
\todo{use the paragraphs below as need}
A key question which \paperTitle answers is, how can contact force, which is a purely mechanical parameter, be linked to RF signal phase. \paperTitle does this by combining RF and mechanical viewpoint of a simple beam model, consisting of two parallel traces, one being ground trace and other being the signal trace, separated by air. 


In RF viewpoint, this is basically a microstrip transmission line with air as substrate, whereas in a mechanical viewpoint this is basically a cantilever beam model. Viewing the sensor as a cantilever beam model allows mapping forces to contact lengths $l_1$, $l_2$ (Fig. \ref{fig:intro_fig}). Viewing the sensor as a microstrip transmission line allows us to map reflected signal phases to the contact locations where the transmission line gets shorted from either ends ($l_1, l_2$, Fig. \ref{fig:intro_fig}). Hence, by forming this connection between RF and mechanical viewpoints, \paperTitle is able to estimate contact force by observing the phase changes due to shorting of transmission line at different locations. 

Further, \paperTitle designs a novel algorithm to detect this phase change accurate to about a degree, which leads to a force resolution of about 0.2 N. The algorithm takes inspiration from how FMCW/UWB systems estimate signal doppler variations, and uses this idea to give an artificial doppler to the sensor by making it switch at certain frequencies. The artificial doppler generated is high enough to make it isolated from any low doppler environmental signals. 
This allows \paperTitle to estimate phase changes super accurately and robust even to dynamic multipath interference, and then map it back to contact force using the cantilever beam model.
However, instead of testing the algorithm with specialized waveforms and ultra-high bandwidths, we show the algorithm working for OFDM based channel estimation to motivate seamless fusion of communication and sensing for this sensing paradigm.

Hence the technical contributions of this paper are
\begin{itemize}
  \item Ideation and fabrication of a novel force sensing paradigm involving transmission lines 
  \item The sensor design is the first one to sense force position and location across the length of the robot
  \item Performing double sided phase measurements from 2 antennas, and a novel algorithm to address the intermodulated harmonics
  \item Performing accurate sensing of phase by isolating reflected signal from the sensor and combating multipath
\end{itemize}

\fi

% \paperTitle hence   in force sensing for surgical robots. The sensor can, in principle, sense as well as locate contact force across the robot body. This is achieved by abstracting the sensor as a transmission line model. A transmission line model is generated by viewing the sensor as a lumped model of continuous impedences, to provide data in a continuum fashion. The signal trace of the transmission line can be wrapped across the robotic manipulator, and ground layer being the inner diameter of the robot.This, in-effect act like an artificial skin for the robot. However, given the size limitations and the flexibility requirements, it is imperative that this sensor should provide wireless reading capabilities. 

% We leverage 2 key insights here, which allows us to create such an artificial skin capable of sensing force across the length. Firstly, by using mechanical models like cantilever beams etc, the force measure can be inferred by estimating the contact length of the flexible outer layer of skin, which has the signal trace of the transmission line, with the robotic surface acting as a ground layer. To estimate this contact length, we measure the contact lengths from the either end of the transmission line. This is done by measuring the phase change in the signal due to this pressing motion, as the signal now travels a lesser length before reflecting back. The second key insight we have here is that, since all the force information is encoded in the phase change of the signal, this sensing modality can be readily integrated with wireless sensing paradigms, which also leverage sensor data information encoded in phase of the signal. To do so, we have antennas on either ends of the transmission line, and we perform wireless measurements of phase change induced onto either end of the transmission line, in order to estimate the force location and force magnitude. For this, we address issues like intermodulation harmonics, clock drift and multipath correction, to estimate the phase changes accurately and precisely.

% Hence the technical contributions of this paper are
% \begin{itemize}
%   \item Ideation and fabrication of a novel force sensing paradigm involving transmission lines 
%   \item The sensor design is the first one to sense force position and location across the length of the robot
%   \item Performing double sided phase measurements from 2 antennas, and a novel algorithm to address the intermodulated harmonics
%   \item Performing accurate sensing of phase by eliminating clock drifts and cancelling multipath
% \end{itemize}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/sensor.pdf}
% \caption{Transmission line (yellow) is wrapped around the robot body and acts like an artificial skin layer. The contact force manifests as phase changes $\phi_1$,$\phi_2$ as the transmission line which was previously open ended is now shorted at two contact points}
% \end{figure}


==> archive/intro_surface_v1.tex <==
% !TEX root = main.tex
% From a larger persdpective where the problem stands and what people have tried
% one paragraph one message
% Dont put multiple messages 

\section{Introduction}


% Contact force is fundamental 
Contact force is a fundamental sensing measure that affects how we interact with the world around us. Humans sense contact force via mechanoreceptors in our skin, which allows us to sense the magnitude and contact location of even the smallest forces \cite{abraira2013sensory}. 
However, in most of our interactions with the digital world, mostly via our smartphones, laptops and tablets, this rich force information is replaced with a simple sense of touch (contact or no contact). 
In other words, we mostly interact with these entities using only a binary sense of whether or not contact has occurred, while the information about the magnitude of the applied contact force is generally lost.


% touch screens can do only multi-level contact sensing, require wired, continuum of surface?
In recent times, Apple and Google have already started exploring force feedback for richer UI experiences \cite{quinn2019estimating}, and the latest iPhones and Apple watches come equipped with a capacitive force sensor \cite{Apple3Dtouch} to provide haptic feedback to the user. Instead of providing the ability for continuum force sensing, which can enable intuitive UIs to control analog variables like volume/brightness, these sensors just provide a multi-level alternative to the traditional press and hold interfaces to perform binary tasks. %However, the force sensing strain gauge is embedded in the capacitive touch screen and provides a few more levels of contact sensing  and cannot enable continuous force sensing on the continuum. 
Furthermore, the next generation of user-interactions for VR/AR interfaces, will necessitate sensing of full contact force information in addition to simple touch. In summary, to harness the full potential of force controlled interfaces, it is required to sense continuum force instead of sensing digitized levels and location of the force to enable variety of applications. \todo{define continnum more precisely it's vague, also showing results with discrete level in your experiments goes against this point}

% robotics none of the above work, and it space contrained, power constrained problem... 
Another significant area where the current lack of continuum force sensing abilities poses a number of challenges, is robotics, and in particular, surgical robotics. Robotic manipulators hold a huge potential in robotic surgeries, where they can go beyond mimicking a human hand and perform far more intricate  surgeries than even possible by an expert human hand. However, unlike touch screens, robotic manipulators do not have space for placing force sensors like load-cells and strain gauges are not accurate, which prohibits them to sense continuum magnitude and location of a contact force that they experience. \todo{make placement an issue}This severely limits the application capabilities of these robots, to an extent that one of the main roadblocks to enabling these precise robotic surgeries is that doctors  can't ascertain if the path taken by the robot is safe or not \cite{alemzadeh2016adverse}. That is,  doctors do not know, whether while doing the surgery, the robot is in contact with some organs/tissues or not, and whether the contact force is appreciable large to hurt the tissue. Hence, there has to be continuum feedback in terms of contact force, as well as contact location sensing to help the doctors in identifying safe operations of the robot.

\begin{figure}[h]
  \centering
    % \placeholder[width=0.3\textwidth]{$l_1,l_2$ figure here}%
    \includegraphics[width=0.5\textwidth]{figures/introfig_v2_cropped.pdf}
  \caption{Applications targeted by \paperTitle: Surgical robots/tools inside the body inadvertently touch other tissues, leading to potential risks which can be avoided via haptic feedback. Finally, force sensitive robotic grippers could open up new automation possibilities.}
  \label{fig:appl}
\end{figure}

\todo{move this paragraph to the related work} 
To address the need of continuum sensing, recent work has utilized sensor arrays of small point sensors to create a macroscopic force sensitive surface\todo{refs}. 
These point sensors can sense forces very accurately, however only do so over a very small force sensitive area, which fails to provide a space continuum.
In order to achieve the required continuum granularity, a large number of these point sensors per unit area are required, which increases the reading latency and power consumption quadratically. 
Given these limitations, these sensing surfaces can not accommodate seamless wireless capability, that is, to communicate the force sensing data over the air they need dedicated micro-controllers, a battery to meet the power requirements and form factor inaccurate RF transceivers.
The sheer amount of electronics required for these solutions is antithesis to the requirements posed by these applications, where doctor might not want to risk electrical discharges to the tissue and harmful chemical leakage from the battery.


To support seamless wireless sensing capability, these sensors need to have the form factor of a smart surface akin to just a small painting which can be hung around, or in form of small stickers which can be stuck in hard to mount places. 
The binary touch based wireless sensing modalities have recently achieved both these goals, with leading research showing touch based sensing ranging from ubiquitous networked smart surfaces \cite{gao2018livetag} to small stickable RFIDs \cite{pradhan2017rio,li2016paperid}.
However, none of these past works could sense beyond just contact/no contact and were totally oblivious to the magnitude of contact force the touch interaction happened with.

% The key enabling technology to achieve this seamless wirelees sensing was to leverage `backscatter sensing', in which instead of having an active RF toolchain with power amplifiers, ADC quantizers and bunch of other electronics, these sensors just had an antenna and a small identification chip, which directly embedded the touch information in the properties of the signal reflected off from the antenna. Hence, the major question answered by \paperTitle is, how can we backscatter force information, rather than just touch. Such  

Ubiquitous battery-free wireless force sensors with minimal power requirements, could hence open up significant possibilities by adding a new dimension to the sensing capabilities of these upcoming smart surfaces. 
One of the major sensing lacuna with the continuum sensing force sensors is that they can not be used with the surgical robots, which have strict form factor and power requirements, in the sense that pose major challenges on how to mount these on the robot, carrying battery to operate inside the human body which has significant medical risks of harmful chemical leakage and capacitative discharges which can in turn harm the human tissues. 
Further, this has limited the advancement of robotic manipulators, which are often unable to relay critical haptic information back to a human teleoperator. 
Force sensing has even been posed as a `Grand Challenge' for further advancement of surgical robotics \cite{burgner2015continuum}. 
Hence, there is a need for a sensing principle which can sense force across the surface of the surgical robot. 
The main goal here is that the sensing principle should, in effect, act like a continuum artificial skin, instead of providing force measurements at discrete points. 
Furthermore, to achieve this elusive goal, such a sensing paradigm should be low-power and wireless, avoiding the hassles of battery requirements and multiple wires running across the surface.

% Worse, not one of these sensing principles is universally optimal. Depending on whether you would want to sense force at the tip, or near the robot-tissue interface, the appropriate choices are strain gauges and force sleeves respectively. 


% Robotic manipulators hold a huge potential in surgery robotics, where they can go beyond mimicking a human hand and perform far more intricate surgeries than possible by a human hand. However, unlike a human hand, these robotic manipulators are completely oblivious to the magnitude of force they touch their environment with.  Hence, there has to be a feedback in terms of continuum contact force sensing to help the doctors in identifying safe operation of the surgical robot inside the human body.

% Sensing touch interactions on surfaces has also attracted a lot of research interest in the wireless sensing community \cite{pradhan2017rio,li2016paperid,gao2018livetag}. The systems have demonstrated detection of gestures/swipes alongside simple touch events on passive surfaces, which have a lot of HCI applications of extending UIs to such passive surfaces. However, these works are limited in the sense that these can't distinguish events wherein a person is touching with higher/lower force, and in a way provide just 1 bit information related to the touch event. 

\paperTitle presents the design, implementation and evaluation of a sensor prototype which can sense force, as well as it's contact location, accurately and continuously throughout the sensor surface and thus address the low-power continuum sensing lacuna with the current force sensors. 
\paperTitle's design consists of two parts, backscatter enabled sensor and wireless reader. 
The key idea of \paperTitle is to make the sensor transduce contact force into phase changes in the reflected RF signal, which is estimated with the precision of a degree by the wireless reader. 
This precision of phase sensing translates to a force magnitude sensing accuracy of about $0.3$ N, combined with an ultra accurate contact location sensing accuracy of $0.6$ mm.
\paperTitle's sensor consists of two parts, the force to phase transduction mechanism and ensuring robust interference-free wireless connectivity. The wireless connectivity ensures that this phase information is embedded in a high speed wireless channel, enabling low-power wireless force feedback. Said differently, instead of generating wireless signals, \paperTitle conveys the force information in the channel of the interference-free reflected signals. Furthermore, \paperTitle is wide-band and works at all frequencies up to 3 GHz, allowing the reader to be WiFi, Radar or even RFID. Such a wireless force sensor can enable safe, battery-free operation of force sensing surgical robots inside the body and can enable the creation of passive force sensitive surfaces. The two broad themes which \paperTitle's sensor design targets are providing haptic feedback for surgical robots, and a smart force sensitive passive surface design which could be used for HCI. 

\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/design_intro.pdf}
  \caption{\paperTitle vs previous touch sensing works: As contact force increases, the top beam bends more and more coming into larger contact with bottom beam. Past work could only sense contact/no contact, being oblivious to contact force}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/phase_to_len.pdf} 
  \caption{Reflected signal phase changes depends on length travelled on the transmission line till getting reflected from the shorting point. Hence sensing phase from either ends ($\phi_1,\phi_2$) allows to sense the contact positions and hence force}
  \label{fig:phase_v_len}
\end{subfigure}
\caption{Force to phase transduction mechanism}
\label{fig:intro_fig}
\end{figure}

A natural question arises as to how can contact force, a mechanical entity, be related to wireless signal phase, which is a RF signal parameter.
To make this connection, \paperTitle fabricates a sensor having 2 parallel beams separated by some air height. 
To relate force and signal phase, this parallel beam sensor has to be viewed from two classical viewpoints from mechanical and RF domain.
That is, from a mechanical viewpoint, the bending of sensor in presence of a contact force is dictated by popular beam bending mechanical models.
From a RF viewpoint, these two parallel beams separated by air acts like a air-substrate microstrip line, which allows us to relate signal phase with the length traveled on the transmissions line.
A confluence of these viewpoints allows \paperTitle to relate mechanical contact force with RF signal phases (Fig. \ref{fig:intro_fig}).
When a force is applied to the top of of the beam the material bends and connects with a bottom, fixed beam that contains a ground trace, short-circuiting the transmission line and reflecting the signals on both ends. As one applies more force, the surface bends further, increasing the length in contact. 
This increased contact length changes the signal phase from both the ends, and hence relating the applied contact force $F$ with the phase changes from either ends of the sensor.

The next challenge is how to communicate this contact point information wirelessly. One way to estimate this could be to generate a RF signal and use it to measure the length at which this short-circuit arises, and then sample/quantize the information and communicate wirelessly using a radio technology like Bluetooth. However, the above overall process would consume significant power and energy, and would make the sensor bulky and hard to attach to the robots. In contrast, \paperTitle combines the communication and sensing of the force into a single paradigm. Our key idea is to equip both sides of the sensor with an antenna which can reflect the signal after traveling some length on the transmission line before encountering the short circuit and reflecting back, in effect encoding the contact information onto reflected phases. Such reflection requires no power, and would simplify the sensor design. Furthermore, we can just use any external radio to send a signal, and the reflected signal when measured by external radio could estimate the length/additional phase traveled before the short circuit.

A natural next challenge is to measure very accurately the reflection properties arising from \paperTitle's sensor. Typically, when an external radio sends signals out in the environment, it receives many reflections back. In this sea of reflections, \paperTitle needs to identify the reflection corresponding to the sensor and measure its properties. To separate the reflection signal from the rest of the reflections, we add a switch, which toggles at a certain frequency, between the antenna and the sensor. The frequency of switching gives the sensor a unique signature and thus enables us to identify the sensor and isolate the reflection's properties. We do so by uniquely corresponding to the sensor via it's signature and support multiple sensors by choosing different frequencies. 

In summary, \paperTitle builds a backscatter tag whose switch switches from no-reflection to the reflection phase dependent upon the force applied. We measure the phase shift on the external receiver to infer the force. \paperTitle forms analog modulation with backscatter communication and enables measurement of the force. Furthermore, \paperTitle supports wide-band operation on the sensor i.e. it can backscatter entire sub-3 GHz, so it can be read by any external radio.
A natural question is how to decode the analog phase information from the sensor. 
For this, \paperTitle designs a novel phase sensing algorithm which just requires periodic channel estimates and can thus work with any wideband channel sensing waveform.
\paperTitle's algorithm views the switching of the signal at the sensor as an artificial-doppler, which allows it to isolate the signal from the environment in doppler domain.
After this separation, \paperTitle's phase sensing algorithm allows to measure the phase changes from the sensor over the entire bandwidth of the signal, which facilitates super accurate phase sensing to accuracy of about $1^{o}$. This gives us a force resolution of $0.3$N, with ultra high contact location accuracy of $0.3$mm. We prototyped \paperTitle using a sensor consisting of a multi-layer beam with a microstrip line attached to the bottom, which, when pressed, contacts a ground trace on a fixed layer below.
%which provide low loss and consumes low power, which is driven by a ring-oscillator implemented on the FPGA. 
The prototyped sensor works for entire sub-3 GHz verified with the vector network analyzer. We used USRP radios as the readers, and tested the sensor at 900 MHz and 2.4 GHz, two most popular ISM bands. We show that the sensor can be read up to 10 meters of range over the air, and show the algorithm working even when the propagation occurs over the gelatin based muscle/fat tissue layers composition similar to the human body to motivate the surgical applications. 

% \todo{agrim I have commented the part below, please feel free to bring it back... }

\if 0
\todo{use the paragraphs below as need}
A key question which \paperTitle answers is, how can contact force, which is a purely mechanical parameter, be linked to RF signal phase. \paperTitle does this by combining RF and mechanical viewpoint of a simple beam model, consisting of two parallel traces, one being ground trace and other being the signal trace, separated by air. 


In RF viewpoint, this is basically a microstrip transmission line with air as substrate, whereas in a mechanical viewpoint this is basically a cantilever beam model. Viewing the sensor as a cantilever beam model allows mapping forces to contact lengths $l_1$, $l_2$ (Fig. \ref{fig:intro_fig}). Viewing the sensor as a microstrip transmission line allows us to map reflected signal phases to the contact locations where the transmission line gets shorted from either ends ($l_1, l_2$, Fig. \ref{fig:intro_fig}). Hence, by forming this connection between RF and mechanical viewpoints, \paperTitle is able to estimate contact force by observing the phase changes due to shorting of transmission line at different locations. 

Further, \paperTitle designs a novel algorithm to detect this phase change accurate to about a degree, which leads to a force resolution of about 0.2 N. The algorithm takes inspiration from how FMCW/UWB systems estimate signal doppler variations, and uses this idea to give an artificial doppler to the sensor by making it switch at certain frequencies. The artificial doppler generated is high enough to make it isolated from any low doppler environmental signals. 
This allows \paperTitle to estimate phase changes super accurately and robust even to dynamic multipath interference, and then map it back to contact force using the cantilever beam model.
However, instead of testing the algorithm with specialized waveforms and ultra-high bandwidths, we show the algorithm working for OFDM based channel estimation to motivate seamless fusion of communication and sensing for this sensing paradigm.

Hence the technical contributions of this paper are
\begin{itemize}
  \item Ideation and fabrication of a novel force sensing paradigm involving transmission lines 
  \item The sensor design is the first one to sense force position and location across the length of the robot
  \item Performing double sided phase measurements from 2 antennas, and a novel algorithm to address the intermodulated harmonics
  \item Performing accurate sensing of phase by isolating reflected signal from the sensor and combating multipath
\end{itemize}

\fi

% \paperTitle hence   in force sensing for surgical robots. The sensor can, in principle, sense as well as locate contact force across the robot body. This is achieved by abstracting the sensor as a transmission line model. A transmission line model is generated by viewing the sensor as a lumped model of continuous impedences, to provide data in a continuum fashion. The signal trace of the transmission line can be wrapped across the robotic manipulator, and ground layer being the inner diameter of the robot.This, in-effect act like an artificial skin for the robot. However, given the size limitations and the flexibility requirements, it is imperative that this sensor should provide wireless reading capabilities. 

% We leverage 2 key insights here, which allows us to create such an artificial skin capable of sensing force across the length. Firstly, by using mechanical models like cantilever beams etc, the force measure can be inferred by estimating the contact length of the flexible outer layer of skin, which has the signal trace of the transmission line, with the robotic surface acting as a ground layer. To estimate this contact length, we measure the contact lengths from the either end of the transmission line. This is done by measuring the phase change in the signal due to this pressing motion, as the signal now travels a lesser length before reflecting back. The second key insight we have here is that, since all the force information is encoded in the phase change of the signal, this sensing modality can be readily integrated with wireless sensing paradigms, which also leverage sensor data information encoded in phase of the signal. To do so, we have antennas on either ends of the transmission line, and we perform wireless measurements of phase change induced onto either end of the transmission line, in order to estimate the force location and force magnitude. For this, we address issues like intermodulation harmonics, clock drift and multipath correction, to estimate the phase changes accurately and precisely.

% Hence the technical contributions of this paper are
% \begin{itemize}
%   \item Ideation and fabrication of a novel force sensing paradigm involving transmission lines 
%   \item The sensor design is the first one to sense force position and location across the length of the robot
%   \item Performing double sided phase measurements from 2 antennas, and a novel algorithm to address the intermodulated harmonics
%   \item Performing accurate sensing of phase by eliminating clock drifts and cancelling multipath
% \end{itemize}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/sensor.pdf}
% \caption{Transmission line (yellow) is wrapped around the robot body and acts like an artificial skin layer. The contact force manifests as phase changes $\phi_1$,$\phi_2$ as the transmission line which was previously open ended is now shorted at two contact points}
% \end{figure}


==> benchmarks.tex <==
% !TEX root = main.tex

\section{Microbenchmarks}
\done{S11-S33 plots and VNA data}\\
\done{To justify sensor's fabricated properly}

To benchmark \paperTitle's sensor design, RF impedance matching and mechanical force versus phase behavior, we first test the sensor with VNA which gives us accurate phase and magnitude measurements for a wide set of frequencies. 
\subsection{Two port circuit analysis of the sensor}

In this experiment, we connect 2 ports of VNA to either end of the sensor and then plot the insertion/thru losses to test 50 $\Omega$ impedance matching of the sensor. From our Ansys HFSS simulations (Fig. \ref{fig:hfss_sims}), we expect that by having the ratio between trace width and sensor height to be around $4:1$, we should get good impedance matching. Hence, we design a air substrate microstrip line with trace width 2.5~mm, ground trace width 6~mm and height as 0.63~mm to come close to the required 4:1 ratio. This gives us S11/S22 below -10 dB over the entire frequency range from 0 to 3 GHz alongwith linear S13 phase which justify the broadband nature of the sensor.

\begin{figure}[H]
  \centering
  \includegraphics[width=0.4\textwidth]{results/s11-s33.pdf}
  \caption{RF propagation characeristics in the sensor. Across the entire 3 GHz frequencies, S11 is below -10 dB, S12 is about 0 dB with linear phase. }
  \label{fig:s11_mag_plot}
\end{figure}

% Finally, with the same setup, we test the phase linearity of the sensor. If the sensor is perfectly matched to $50 \Omega$ we would get a linear relationship between the length signal travels on the sensor and phase. Hence, to test it, we touch the sensor at equispaced points and plot the S11 and S22 phases. We expect the 

\subsection{Mapping Force versus Phase profile}
Next, we attempt to characterize the relationship between phase and force by applying certain forces to the sensor, noting the phase values on the either ends of the sensor (i.e. S11 and S22 phases), and finally plotting the force versus phase profile to understand how phase would vary as force is increased. For this, we have an experimental setup consisting of an actuator to apply the force on the sensor, a load cell to measure the ground truth force reading, and an Arduino to read the load cell output and command the actuator to apply a certain level of force. 

% \begin{figure}
% \centering
% \includegraphics[width=0.5\textwidth]{figures/vna_expmt_temp.png}
% \caption{VNA Testing Setup}
% \end{figure}

First, we show the S11/S22 phase versus force plots for 3 chosen locations, which are chosen to be 20~mm, 40~mm, 60~mm for a sensor which is 80~mm long. This would describe the general behavior of the sensor at the left end, center and right end of the sensor and would verify the Comsol simulations discussed in Section \ref{section:sim_comsol}.

\textcolor{magenta}{\textbf{Cedric: I can help with this part as related to mechanical behavior validation and modeling}}


\begin{figure*}[ht]
\begin{subfigure}[t]{.33\textwidth}
  \centering
  % include first image
  \includegraphics[width=.9\linewidth]{results/20mm_VNA_2400.pdf}
  \caption{Force vs Phases, contact point: 20mm}
  \label{fig:vna20}
\end{subfigure}
\begin{subfigure}[t]{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{results/40mm_VNA_2400.pdf}
  \caption{Force vs Phases, contact point: 40mm}
  \label{fig:vna40}
\end{subfigure}
\begin{subfigure}[t]{.33\textwidth}
  \centering
  % include second image
  \includegraphics[width=.9\linewidth]{results/60mm_VNA_2400.pdf}
  \caption{Force vs Phases, contact point: 60mm}
  \label{fig:vna60}
\end{subfigure}
\caption{VNA testing results for force vs Port1, Port2 phases}
\label{fig:vnaplots}
\end{figure*}

\subsection{Sensor Model Benchmarks}
Finally, after verifying the force profiles predicted by comsol, we use the same VNA setup to collect the profiles at additional locations, in order to create a sensor model which goes from measured two-sided phases to force magnitude and force location. After collecting this data, we interpolate at the intermediate locations, which allows us to create a force vs 2-sided phase heatmap and force location vs 2-sided phase heatmap, as shown below. As we expect, the force location heatmap turns out to be rather linear, since we have matched the sensor impedance to 50 $\Omega$. The force magnitude heatmap is rather non-linear since it is governed by cantilever beam bending models which are slightly more involved than a simple linear relationship.

\begin{figure}[H]
  \centering
    \placeholder[width=0.3\textwidth]{4 plots, $\phi_1, \phi_2$ vs Force and $\phi_1, \phi_2$ vs Force locations heatmap at both 900M,2400M Status: \notdone{ToDo}}
  \caption{Phase vs Force/Force Location heatmap, as measured by the VNA}
  \label{fig:force_phase_plot}
\end{figure}

% To understand the generality of the model and the errors introduced at intermediate locations via interpolation, we repeat the test at an intermediate location ($35$ mm), and compare the ground truth readings by the VNA and the estimates predicted by the model.

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{2 plots, showing S11/S33 phase, interpolated estimates versus force at intmd location 35mm. Status: \notdone{ToDo}}
%   \caption{Phase vs Force profile at intmd locations, as measured by the VNA}
%   \label{fig:force_phase_plot_intmd}
% \end{figure}

% As we observe from Fig. \ref{fig:force_phase_plot_intmd}, our model compared sufficiently well against the ground truth data collected at an intermediate location, which confirm the generality of the model.
 
% The sensor was evaluated to confirm and test the following principles
% \begin{itemize}
% 	\item \textbf{Force Transduction Mechanism}, which utilizes cantilever beam model to map force to contact lengths
% 	\item \textbf{Mapping contact lengths to Phase changes}, using the transmission line model
% 	\item \textbf{Sensing phases from either end of the sensor}, by utilizing diode non-linearities
% 	\item \textbf{Wireless sensing of phases with sensor placed inside tissue phantoms}, by evaluating the best frequency for in-body propagation and applying appropriate CFO/channel correction
% \end{itemize}

% \subsection{Force Transduction Mechanism}
% By utilizing ... cantilever theoretical constructs, We derive the relationship between force $F$ and contact lengths $l_1,l_2$, given by

% \begin{equation}
% F = f(l_1,l_2)
% \label{eq:force_vs_len} 
% \end{equation}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.3\textwidth]{figures/fvl.pdf}
% \caption{The applied force $F$ can be related to contact lengths $l_1$, $l_2$ via Eq. \eqref{eq:force_vs_len} (This image should be replaced by an image of the testing setup here)}
% \end{figure}

% To experimentally verify this equation, we utilize a setup consisting of a copper strip emulating a cantilever beam, and a potentiometer. An actuator applies force to the copper strip, and the ground truth value of the force is measured via the <actuator feedback, weighing scale?>. The experimental results are shown in Fig. \ref{fig:force_vs_len}.

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Force vs $l_1, l_2$ graph here}%
%   \caption{Maybe 4 subplots, each having different $l_1$, $l_2$. We plot the expected theoretical values in dotted lines and obtained results in solid lines to motivate Eqn \eqref{eq:force_vs_len}}
%   \label{fig:force_vs_len}
% \end{figure}

% \subsection{Mapping contact lengths to Phase changes}

% Hence, to sense contact force, we need to sense $l_1$, $l_2$ here. We do this by modeling the sensor as a transmission line, and make an observation that $l_1, l_2$ can be linked to phase changes in the reflected signal of the transmission line. Recall that $\Delta \phi = \frac{2\pi}{\lambda} \Delta L$, i.e. phase change of the signal is given by $2\pi$ times the fraction of wavelength traveled. When we press with force $F$, $\Delta L = l_1, l_2$ respectively when measuring from either end of the sensor. Hence, we get 

% \begin{equation}
% \phi_1 = \frac{2\pi}{\lambda} (l_1), \phi_2 = \frac{2\pi}{\lambda} (l_2)
% \label{eqn:phi_v_l}
% \end{equation}
% A caveat here is that the relationship between phase change and length is linear only if impedances match and their are no interface reflections causing non-linear phase changes. For this, it is imperative that the sensor strip length and spacer gap is chosen such that $50 \Omega$ is matched. To evaluate this We test the phase response of the sensor via VNA. A linear phase plot like as shown in Fig. \ref{fig: lin_phase_resp} confirms that the sensor is properly impedance matched and hence Eqn \eqref{eqn:phi_v_l} hold true.

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Phase vs Frequency or Calculated length from VNA experiments here}%
%   \caption{Linear phase response measured by VNA to motivate Eqn \eqref{eqn:phi_v_l}}
%   \label{fig:force_vs_len}
% \end{figure}

% \subsection{Sensing phases from either end of the sensor}
% Now that we have established relation between force and $\phi_1, \phi_2$, we now evaluate our strategy to sense these $\phi_1$, $\phi_2$ wirelessly. A naive strategy here would be to have two antennas on the either ends, and do TDMA between the two ends to sense $\phi_1, \phi_2$. However, keeping in mind the passive nature of the sensor, and the size requirements as well, a better strategy would be to somehow do testing with just a single antenna. We leverage a key insight that by utilizing a diode on one end of the sensor, we can modulate information about phase from that end on the higher harmonics. After estimating this phase from higher harmonics, we can then go back to the first frequency and solve or the phase from the other end. This is visually illustrated below.

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/Selection_480.png}
% \caption{Performing double ended phase sensing with help of non linear circuit elements}
% \end{figure}

% To evaluate this, we proceed in steps. Firstly, we just test if indeed we are getting these harmonics or not. We do this by attaching antenna to the switch, and grounding the diode, visually illustrated in the below figure.

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/Selection_481.png}
% \caption{Harmonics test setup}
% \label{fig:test_harmonics}
% \end{figure}

% We transmit a sinusoid tone at $f_c$ via the transmitter. If the hypothesis that diode, along with the switch would give out harmonics like $f_c\pm f_s, f_s\pm 3f_s, f_c\pm 5f_s$, we would observe the following spectrum.

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Received spectrum by the test configuration in Fig. \ref{fig:test_harmonics} }%
%   \caption{Spectrum plot}
%   \label{fig:expmt_harmonics}
% \end{figure}

% The presence of harmonics confirms the fact that we get the harmonics due to non-linear characteristics of the diode. We then proceed on testing if we can indeed sense $\phi_1, \phi_2$ via this mechanism. 


% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Force vs $\phi_1, \phi_2$ graph here, generated by wireless testing over the air}%
%   \caption{Maybe 4 subplots, each having different $\phi_1$, $\phi_2$. We plot the readings obtained by testing setup with potentiometers and with the wireless diode testing setup to motivate wireless sensing}
%   \label{fig:wireless_ota}
% \end{figure}

% \subsection{In-Body testing}

% Finally, we motivate testing of the sensor when placed inside the body. To emulate EM properties of human body tissues, we make artificial tissue phantoms using <cornflour, vegetable oils etc>.

% We first figure out the best frequency for such in-body propagation, by testing out antennas of various size and frequencies and characterizing their propagation losses inside these tissue phantoms.

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Propagation loss vs Frequency plots here}%
%   \caption{Figuring out the best frequency of operation inside body}
%   \label{fig:force_vs_len}
% \end{figure}

% The sensor readings would be hampered due to severe attenuation etc from the in body propagation. We perform <some CFO/multipath> correction algorithm explained in the technical section to mitigate these effects. We see that placing the sensor inside the body doesn't affect the wireless readings much, as the force readings and accuracy is largely similar.

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Force vs $\phi_1, \phi_2$ graph here, generated by wireless testing inside tissue}%
%   \caption{Maybe 4 subplots, each having different $\phi_1$, $\phi_2$. We plot the readings obtained by with the wireless diode testing setup, placed inside body and the same setup over the air to motivate wireless sensing works even when sensor is obstructed by tissues etc}
%   \label{fig:wireless_tissue}
% \end{figure}

==> design.tex <==
% !TEX root = main.tex

\section{Design}
% force to length
% length to phase
% go about how to measure this phase
% Process: Wireless Reader outside, surfae continuum press on it, detect point+force. This information done 
% while being low power. Sensing/Commn component. Sensing thus is dependent on multipath/SQ/
% Intro like the organization, 

% At heart of WiForce lies  key design components which allow it to sense contact forces wirelessly with low power consumption and minimal electrnics requirement. 
% Fig.~\ref{fig:design_overview} illustrates the design overview of WiForce.
% \todo{you are killing all the surprises in the paper here itself, not going in detail...}
% \todo{this can be background and motivation section, where you explain why you need to make it low power and electronics less, here the requirements and solutions are muddled up and things presents without excitement...}
% \todo{I don't like the writing of this section, it is very non-linear you didn't explain me the phase and how phase can get force and jumped direclt to wireless part}

% At the heart of WiForce lies the key design principle of using minimal electronics to enable sensing with extremely low power consumption. 
% We therefore follow the design principles of backscatter communications, where instead of generating and transmitting the wireless signal, which requires various circuit components like mixer, LNA and high frequency clock sources, WiForce leverages altering the phase of the reflected signals in order to communicate information about contact force. 
% However, wireless signal phase is a very fickle entity, easily corrupted by timing offsets, hardware non-idealities and multipath effects. 
% Hence, as a first step towards building such a passive force sensor, WiForce designs a robust algorithm to isolate sensor's signals from the environmental clutter which allows for accurate wireless phase sensing. 

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Design overview figure here}%
%   \caption{Fig. summarizing the whole design}
%   \label{fig:design_overview}
% \end{figure}


% When interacting with the sensor, the contact locations from either end of the sensor can be linked to contact force by which the sensor is being interacted with.  

% WiForce uses the popular technique of on-off keying modulation of the reflected signal, via a RF-switch to isolate the reflected signal from the LOS signal. 
% Performing two-ended sensing with naive on-off keying modulations, with the requirement of frequency and time isolations, poses issues with inter-modulation and phase discontinuity. 
% To resolve this, WiForce designs a novel clocking strategy which isolates the two ends electrically to reduce inter-modulation, at the same time preserving frequency isolation, which allows reflected phases to be read independently from both the ends of the micro-strip line.

% Finally, equipped with the force sensing micro-strip line prototype and two-ended backscatter solution, WiForce designs a wideband sensing algorithm to isolate the sensor reflected signal from the ambient multipath signals, in order to perform very accurate phase change measurements. 
% WiForce's sensing algorithm borrows elements from doppler sensing algorithms traditionally used with FMCW/UWB radar system. 
% The key insight here is that the on-off keying gives the sensor an artificial doppler which can then be sensed via these traditional doppler sensing algorithms. 
% However, instead of utilizing hardware intensive solutions like FMCW/UWB, we show that equivalent algorithms can work in-general with any wideband channel estimation strategy, and as a demonstration, we showcase this with a simple OFDM based channel estimation method.
% On the other hand, the sensor height plays a more crucial role here, affecting both the force transduction mechanism and RF impedance matching, which requires a careful 
% Force sensing mechanism
% Phases to Forces

% OFDM: Can get in implementation
% S11 figure (Fig. 9) can go in implementation
% Justify the sensor design

\subsection{Force Transduction Mechanism}
\label{section:force_transduction}
The first natural question which the WiForce's design tackles is, how can contact force, a purely mechanical quantity, be linked to reflected signal phase, a RF signal parameter. 
The aim in doing so, is that if such a relationship can be created, force information can be sensed simply by backscattering RF signals, enabling low power wireless force sensing.
Hence, to do so, WiForce connects the classic concepts of RF transmission line and beam mechanics to design a sensor prototype which can communicate contact force magnitude and location over the reflected signal phase. 
The trick to do so lies in understanding that the same sensor, having two parallel traces separated in air using spacers, can be viewed as a beam that is bending from a mechanical viewpoint and as a microstrip line from a RF viewpoint.
\begin{figure}[h]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/transduction_imga.pdf}
  \caption{Beam Bending: Shorting points shift further apart as the force magnitude increases}
  \label{fig:transductiona}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/transduction_imgb.pdf}
  \caption{Phase Changes due to Beam Bending: Phase-force profiles for the three scenarios above obtained via VNA experiments}
  \label{fig:transductionb}
\end{subfigure}
\caption{ \done{\%\% REVIEW \%\%}The shifting of shorting points due to increased force changes the reflected phase on both the ports, and depending on the location where force is applied both the ports different phase-force profiles.}
\label{fig:transduction}
\end{figure}
The confluence of these two viewpoints results in an interesting relationship between contact force and reflected signal phase.
When a contact force $F$ is applied on the sensor, the top beam bends in accordance with beam mechanics models, which leads to different contact locations with the bottom beam as the force increases.
From a RF transmission line viewpoint, this bending causes different shorting points between the top beam, which is the signal trace, and the bottom beam, which is the ground trace.
As the shorting points on the sensor change, so do the phases accumulated by the propagating signal from both ends, as the signals travel less distance on the microstrip line before getting reflected at the shorting points.

In accordance with beam mechanics models, the top beam bends and touches the bottom beam under application of a force. As this force increases, the beam gets pressed and deforms even more, leading to an increased contact length with the bottom beam, which moves the shorting points farther away from each other (Fig.~\ref{fig:transductiona}). Since the shorting points get farther apart, the increased force magnitude induces different phase changes on either ends of the sensor. This is because the signals travel different lengths on the transmission line before getting reflected. This effect manifests itself in the form of a varying phase-force profile depending on the point of application of the contact force (Fig.~\ref{fig:transductionb}). When the contact force is applied at the middle of the sensor, both ports show a symmetric phase change since the shorting lengths move symmetrically. However, when force is applied towards the ends of the sensor, the part of beam closer to the point of application being more sensitive shows more shift in the shorting points, whereas the farther side of the beam essentially saturates and doesn't show much pronounced phase changes (Fig.~\ref{fig:transduction}). 

% From the cantilever beam bending models, the beam bends differently if the forces are applied on the ends of the sensor, as compared to forces applied towards the middle of the sensor. In fact, there is a one-to-one relationship between the applied force location and the initial shorting point on the sensor, i.e. 

% % \subsubsection{Contact Force and sensor shorting lengths}
% % 3d, new dimesnion
% A number of past works have used micro-strip lines to create backscatter/RFID based touch sensors to infer touching points along the length of the sensors~\cite{li2016paperid,pradhan2017rio,gao2018livetag}. 
% However, all of these were either printed on a paper, or had a very thin fixed height solid substrate. 
% WiForce adds a new dimension in design of such sensors, by prototyping micro-strip lines with air as substrate, which allows interaction not only along the length, but also height (Fig.~\ref{fig:design_intro}).

% \begin{figure}[h]
%   \centering
%     \includegraphics[width=0.5\textwidth]{figures/design_intro.pdf}
%   \caption{WiForce vs past RFID based touch sensing works: The vertical separation and capability for two-ended sensing allows WiForce to estimate not only the touch location, but also the contact force}
%   \label{fig:design_intro}
% \end{figure}

% This added vertical dimensionality manifests itself as two-ended touch sensing, i.e., due to the vertical air separation between the ground and signal trace, the applied contact force is related to the shorting lengths on either ends. 
% This relationship is governed by traditional mechanical models pertaining to how a cantilever beam deforms under application of a contact force. 
% As the beam starts deforming more and more as the applied force increases, more of the signal trace comes into contact with ground trace, which changes the shorting lengths on either ends. 
% Finally, the reflected signal phase would depend on how much did the signal travel before getting reflected from the shorting point. 
% Hence, ultimately, by sensing phase changes from the either ends of the microstrip line WiForce can sense more than just binary touch, but also the contact force by which the touch interaction occurred.  

% \input{mech_design.tex}

\subsection{How to Sense Force Wirelessly?}
\label{Subsec:double-ended}
Sensing these phases from either side of the sensor can be done by using a VNA to perform $2$-port analysis of the sensor and noting the S11-S22 phases due to these shorting points. 
However, performing the same task wirelessly is far from trivial, since phase of a wireless signal is easily corrupted by timing offsets, hardware non-idealities, and multipath effects. 

Further, the concept of obtaining absolute phase is challenging as well, since any wireless phase measurement would also account for the phase which the signal accumulates by traveling some distance over the air. 
This challenge is only exacerbated when the signal whose phase we are interested in is a backscattered signal. That is, the signal is not generated at the sensor, but instead is the reflection of an excitation signal sent by the transmitter, undergoing absorption/reflection losses at the sensor and also traveling more distance than the direct path excitation signal. 
The receiver here has to read the phase of the backscattered signal, under the presence of a much stronger excitation signal. 
So, how does WiForce actually perform wireless sensing of the phase changes due to contact force, given all these challenges?

The first key idea which allows WiForce to first isolate the reflected signal from the excitation signal, as well as the environmental clutter, is to modulate the reflection with a simple power efficient On-Off Keying (OOK) strategy. 
This basically shifts the frequency of the excitation signal after reflection, allowing the reflected signal to be recovered in the frequency domain. 
The second key idea, which gets rid of phase accumulation over the air as well as some constant phase offsets from static multipath/hardware non-idealities, is that the contact force information is actually present in the `differential-phase' and not the absolute phase. 
That is, by just observing phase jumps at the shifted frequency signal, one can infer how much contact force actually caused this phase jump. 

\begin{figure}[h]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/one_ended_figa.pdf}
  \caption{Before force is applied}
  \label{fig:contactlengtha}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/one_ended_figb.pdf} 
  \caption{After force $F$ is applied}
  \label{fig:contactlengthb}
\end{subfigure}
\caption{ \done{\%\% REVIEW \%\%}Sensing contact length via backscatter phase: modulating with a square wave (blue) allows isolating from reflected signal from the excitation signal in frequency domain. Observing differential phase ($\angle r_1(t)-\angle r_2(t) = \phi_{\text{full}}+\cancel{\phi_{a}}-\phi_{\text{touch}}-\cancel{\phi_a}$) allows to get rid of phase accumulated over the air (cyan) and gives a measure of the contact length $l_1$.}
\label{fig:contactlength}
\end{figure}

This strategy to sense phase jumps from backscatter signals is visually illustrated in Fig.~\ref{fig:contactlength}. 
There are three key components to the design of WiForce's sensing modality. 
First, WiForce performs OOK by utilizing square waves to modulate the reflected signal in order to isolate it from the excitation signal. 
The tag receives the excitation signal $s(t)$ and reflects $s(t)m(t)$ where $m(t)$ is a square wave. 
Consider 
$$m(t) = \begin{cases} 0, nT\leq t< (nT+\frac{T}{2}) \\ 1, (nT +\frac{T}{2})\leq t< (n+1)T, n\in \mathbb{Z} \end{cases}$$
Expanding $m(t)$'s Fourier series, we get a sum of odd harmonics
$$m(t) = \sum_{k\in (2i+1), i\in \mathbb{Z}} \frac{1}{|k|}e^{(j2\pi kf_st)}$$ where $f_s=\frac{1}{T}$. 
Ignoring the weaker high order harmonics, we get reflected signal as $r(t) = s(t)m(t) \approx s(t)e^{j2\pi f_s t}$. 
Hence the reflected signal will be shifted by frequency $f_s$, corresponding to the time period of the modulating square wave. 
This allows the reflected signal, $r(t)$, to be isolated from the excitation signal, $s(t)$, in the frequency domain, since the reflected signal would appear to be shifted in frequency. 

% The strategy of using clocked RF switches to do so has been explored by multiple papers \notdone{CITE}.
% \margins{I think making the bottom half of each subfigure (ie the sensor and switch etc) larger (full column width) would help. Right now it's too small. Then you can decrease size of transmitter and receiver. Also, green and red signals are hard to see on top of the colored sensor. Maybe make sensor grey.}
After isolating the reflected signal from the excitation signal, WiForce reads the phases at shifted frequencies, and observes the phase jumps caused by the shifting of contact edges between the traces due to an applied force. 
Let us denote the reflected signal just before a contact force was applied as $r_1(t)$. 
In addition to getting modulated by the square wave, $r_1(t)$ would accumulate phases due to traveling over the air ($\phi_a$), as well as along the entire length, $L$, on the microstrip line sensor ($\phi_{\text{full}}$) (Fig.~\ref{fig:contactlengtha}). 
Hence, $\angle r_1(t) = \phi_{\text{full}}+\phi_a$. 
Now we denote the reflected signal after a contact force $F$ is applied to the sensor as $r_2(t)$, which shorts the microstrip line at some location $l_1$. Assuming that the sensor doesn't move significantly between the instantaneous time points before and after application of forces, we have $r_2(t)$ also accumulating phase $\phi_a$ and accumulating phase $\phi_{\text{short}}$ due to traveling until the short location. 
Hence, $\angle r_2(t) = \phi_{\text{short}}+\phi_a$. 
Thus, the differential phase between $r_1(t), r_2(t)$ would be $\phi_{\text{full}}+\cancel{\phi_{a}}-\phi_{\text{short}}-\cancel{\phi_a}$, and thus the differential phase jump would give us $\phi_{\text{full}}-\phi_{\text{short}}$. 

Since $\phi_{\text{full}}$ is the net phase accumulated by the signals by traveling the full length of the microstrip line, this is a fixed quantity which can be obtained beforehand from accurate VNA readings. Thus, reading the differential phase allows us to estimate  $\phi_{\text{full}}-\phi_{\text{short}}$, and in turn, $\phi_{\text{short}}$, which is the phase due to the shifting of contact points caused by an applied force. However, we need to sense this phase jump from not just one end, but also from the other since the applied force depends on both these phases. A natural solution is to have RF switches on both ends of the sensor, to toggle them at different frequencies ($f_{s_1}/f_{s_2}$), and to read the phase jumps at these shifted frequencies. Further, to ensure that reflection occurs similarly to how it did with one ended sensing, the design can utilize `reflective-open' switches, which have ports as open reflecting ends when the ports are switched off.

Although this solution to sense phase jumps from both ends is correct in spirit, there is more to the double-ended sensing problem than just naive frequency multiplexing. Recall that sensing differential phases requires sensing the phase before force was applied, in which the sensor acts like a through line between the two ends. Hence, if both the switches are toggled-on, the signals will just go through and not reflect anywhere and leak out from the other end. This will cause intermodulated reflections, where the reflected signal would be partially modulated by both the RF switches. This is visually illustrated in Fig.~\ref{fig:intermod}.


\begin{figure}[b]
\centering
\includegraphics[width=0.45\textwidth]{figures/intermod.pdf}
\caption{\done{\%\% REVIEW \%\%}By giving different frequency clocks to the two switches, there would be overlap times (red shading) where both switches are toggled on, which would cause intermodulation as the signal will leak through instead of getting reflected.}
\label{fig:intermod}
\end{figure}

Hence, the question to be posed is, how to avoid this intermodulation issue? When one switch is toggled-on to connect to the sensor, the other switch has to be toggled-off to act like an open reflector, in order to avoid the intermodulation outputs. By observing this, a naive attempt would be to consider time multiplexing instead. That is, at a given time only one switch toggles and the other is terminated, and after a definite time slot the roles reverse. However, this would then complicate the differential phase algorithm since it would be required to track the phase jumps arising due to clocks turning on and off. Further, it would limit the potential usage of multiple such sensors, since this time scheduling has to be agreed upon over multiple of these sensors.
To bypass these issues, WiForce presents a unique clock design which would avoid the intermodulation issue and at the same time provide frequency separation for the reflected signals coming from either end.


The unique insight which allows WiForce to have such a clock scheme is the use of duty cycle properties of square wave Fourier series. In a standard square wave, with $50\%$ duty cycle, all the even harmonics (i.e. every second harmonic) are absent. Similarly, in a wave with $25\%$ duty cycle, every fourth harmonic would be absent. Hence, a frequency $f_s$, $25\%$ duty cycle square wave will give modulation at $\underline{\mathbf{f_s}},2f_s,3f_s, 5f_s, 6f_s, 7f_s, 9f_s \ldots$ \notdone{\%\%Not sure if mathematical proof is required here\%\%} Similarly, a frequency $2f_s$, $25\%$ duty cycle square wave will give modulation at $2f_s,\underline{\mathbf{4f_s}},6f_s,10f_s\ldots$ Observe that a combination of these 2 clocks will cause interference at $2f_s$, but can be read up individually at $f_s$ for the former clock, and $4f_s$ for the latter clock. Hence, a combination of these 2 clocks can provide separation in the frequency domain. Also, by controlling the initial phases of these two clocks, we can suppress the intermodulation problem as well. This is possible because when one clock is high, the other clock will be guaranteed to be low and vice versa (Fig.~\ref{fig:two-sided}). Hence, at any given time, only one port will be on, and other port will be reflective open. Also, since the clocking strategy provides separation in the frequency domain, we can add them via a splitter to enable double-ended sensing with just one antenna. Thus, we can read the differential phases at $f_s, 4f_s$ due to new shorting points caused by the bending of the sensor under an applied force $F$.
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figures/two-ended.pdf}
\caption{\done{\%\% REVIEW \%\%} The two-ended sensing approach of WiForce. Observe that at any time instant, only one port is connected to the sensor, the other port is reflective open.}
\label{fig:two-sided}
\end{figure}

\subsection{Rejecting Multipath by Reading Forces at Multiple Frequencies}
\label{Subsec:wideband}

By utilizing the clock design strategy discussed, phases from both ends of the sensor are modulated with different shifted frequencies, which distinguish them from the excitation signal which is received directly without any frequency shifts. 
Hence, the next step in WiForce's design is to formulate an algorithm which can sense these phases accurately.
WiForce leverages a wideband excitation signal, which enables the reading of these phase changes at multiple frequencies and the harnessing of averaging gains. 
% In contrast, most of the past phase sensing solutions for RFID based touch sensing have largely used narrowband sensing, which further require a specialized RFID reader~\cite{pradhan2017rio}, whereas WiForce's solution can work with commodity 
Thus, WiForce first comes up with a strategy to sense these phases from periodic channel estimates. 
By doing so, WiForce's strategy becomes waveform-agnostic, and can be used in general with any wideband sensing waveform that allows for periodic channel estimates, such as FMCW/UWB/OFDM and more.

WiForce's strategy consists of two steps. The first step is to detect the reflected signal from the sensor, which is basically a backscattered excitation signal modulated by a square wave, giving it a frequency shift. 
An important connection to make here is that this frequency shift originating from square wave modulation can be alternately viewed as an `artificial-doppler', since doppler effects also introduce similar frequency shifts.
Hence, the first step in WiForce's algorithm is to utilize an FFT-based technique of sensing these frequency shifts, which works very similar to how doppler is traditionally sensed via wideband sensing waveforms like FMCW and UWB. On a similar vein,~\cite{josephson2019rf} also views the square wave modulation in backscatter tags as an artificial doppler, however, instead of using costly UWB radars, we show that a similar algorithm works with a lower bandwidth OFDM based channel sounding approach. 
Since force information is in the form of phase changes that get rid of the air phases, we don't really require absolute time-of-flight measurements, which need more involved FMCW/UWB based solutions. 

\notdone{\%\% The next few lines motivate the sensing strategy can be used in intro as well, just writing it here to put these thoughts into words \%\%}
Also, making the sensor design work with OFDM-based channel sounding provides interesting opportunities for communication and sensing to co-exist and allows for seamless future integration with Wi-Fi-based solutions. Further, in doing so we introduce a paradigm shift in backscatter sensing solutions, wherein, we don't require the quantization of data into bits and the sending of them over a low throughput link, but the data is instead embedded in the phase differences in channel estimates, and can be read continuously at the receiver. The former strategy requires presence of low power ADCs/data buffers to quantize and communicate the data, in addition to RF switches to isolate the reflected signal from excitation signal, whereas our solution just requires RF switches toggling with a certain clocking strategy. To justify the usage of these ADCs/data buffers, the former strategy requires presence of an explicit wake-up signal so that these power hungry components are used only for a fraction of time. In comparison, our design does not require the presence of such wake-up signals and can be turned-on all the time. Hence, we believe this sensing paradigm would pave the way forward to ultra low-power backscatter sensing links, which can work even in challenging environments like inside body tissue, where the efficiency of RF harvesters might not be able to support the sensing paradigms requiring ADCs/data buffers. \notdone{\%\% End of sensing motivation block\%\%}

% Hence, now we will present how WiForce uses OFDM channel sounding to read the phase changes coming from either end of the sensor. 
\begin{figure*}[h]
\centering
\includegraphics[width=0.95\textwidth]{figures/ofdm_design.pdf}
\caption{WiForce's sensing algorithm which utilizes wideband channel estimates to isolate the signal from multipath in doppler domain. Finally, by grouping the channel estimates into `phasegroups', WiForce can read phase changes over multiple subcarriers which allows for averaging gains to make the phase sensing robust and accurate}
\label{fig:ofdm_expl}
\end{figure*}

Hence, now we will present how WiForce uses channel estimates to read the phase changes coming from either side of the sensor. Since the algorithm requires just the periodic channel estimates, it can work in general with any waveform which can be used to estimate channel.  The algorithm is visually illustrated in Fig.~\ref{fig:ofdm_expl}

Say we are estimating the channel periodically after every $T$ seconds, with frequency steps of $F$ (this could be subcarrier spacing/sweep step in OFDM/FMCW based waveforms). We denote $H(kF,nT) = H[k,n]$ where $k$ is subcarrier index and $n$ is time index. Now, if there are $M$ multipaths in addition to the signal coming from the sensor, we can write the channel estimates as
\begin{equation}
H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + (s_1(nT) e^{-j\phi^1_n}+s_2(nT)e^{-j\phi^2_n})\alpha_s e^{-j2\pi k F \frac{d_s}{c}}
\end{equation}
Here, $\alpha_i$ is the attenuation factor for the $i$-th path, $d_i$ is the distance separation between the TX-reflector and reflector-RX, and $\phi^1_n, \phi^2_n$ is the phase accumulated from the RF propagation in the microstrip line sensor at time index $n$ from sensor end $1$ and sensor end $2$. $s_1(t),s_2(t)$ are the double-ended sensor modulation as per the duty cycled clocking strategy discussed earlier. Expanding them as harmonics, we get $s_1(t) = \sum_{p\neq 4q, q\in \mathbb{Z}} a_p e^{j2\pi pf_{s_1}t}$, $s_2(t) = \sum_{p\neq 4q, q\in \mathbb{Z}} a_p e^{j2\pi pf_{s_2}t}$. We have $f_{s} = f_{s_1} = 0.5f_{s_2}$ and thus modulations at $f_{s}, 4f_{s}$. Ignoring the higher harmonics and the constant factors $a_p$ associated with the Fourier expansion for brevity, we get
% \begin{equation}
% \resizebox{0.45\textwidth}{!} 
% {
%     $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})$
% }
% \end{equation}
\begin{equation}
\begin{split}
 H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} +&  \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+\\ &e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})
 \end{split}
\end{equation}

Now, to isolate the signal coming from the sensor, we take FFT over the $n$-th index, to obtain $\tilde{H}[k,f]$. We observe $N$ channel snapshots and take the following transform:
\begin{equation}
\tilde{H}[k,f] = \sum_{n=1}^N H[k,n] e^{-j2\pi f n T}
\end{equation}

Observe that for this transform, the nyquist frequency would be $\frac{1}{2T}$, and hence, $f_s$ has to be chosen such that $4f_s \leq \frac{1}{2T}$. Hence, assuming $\phi^1_n, \phi^2_n$ stay constant over the period of $N$ snapshots, at $f_s$, $4f_s$, we have,
\begin{equation}
\begin{split}
\tilde{H}[k,f_s] &= \sum_{n=1}^N H[k,n] e^{-j2\pi f_s n T} = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^1_n}\\
\tilde{H}[k,4f_s] &= \sum_{n=1}^N H[k,n] e^{-j2\pi 4f_s n T} = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^2_n}\\
\end{split}
\label{eqn:sensharmonics}
\end{equation}

This draws a parallel to how doppler is sensed from wideband sensing algorithms, and switching in fact gives the sensor an `artificial doppler' which can be sensed as done above. The switching frequency $f_s$ can be related to an equivalent doppler, $f_s = \frac{f_c v}{c}$, and thus an object in the environment moving at velocity $v = \frac{c f_s}{f_c}$ would create interference with the sensor signal. However, the chosen $f_s$ is large enough so that this equivalent speed is so high that it wouldn't appear in the environment for the use cases considered. Hence, taking this FFT isolates the signal coming from the sensor and nulls out the multipath clutter in the environment. 

Recall that while writing Eqn.~\eqref{eqn:sensharmonics}, we assumed $\phi^1_n, \phi^2_n$ stay constant over the period of $N$ snapshots. Basically, this assumes that the force acting on the sensor stays almost constant for about $N$ snapshots, which is a reasonable assumption given it requires some time for mechanical beams to relax and get to steady state under the action of force. Said differently, wireless sensing occurs at much higher sampling rate (about order of MHz), whereas the mechanical forces are much slower (take about 0.5-1 seconds to stabilize). 

Thus, WiForce designs an algorithm to sense these phase differences from the filtered harmonics, and ultimately map them to applied force. The algorithm divides the channel estimates into groups of $N$, referred to as `phase-groups'. For each phase-group we first take the harmonics FFT as described earlier and obtain $2$ $K\times1$ vector from Eqn.\ref{eqn:sensharmonics} for FFT frequency $f_s$, $4f_s$. Assuming there are $N_g$ such phase groups, and for all $N$ samples of $g$-th group, $\phi^1_n,\phi^2_n \approx \phi^1_g \phi^2_g \forall n \in \{1,2,\ldots N\}$. The output at $g$-th phase group, $k$-th subcarrier, after harmonics FFT at $f_s, 4f_s$, is denoted as $P_1[k,g],P_2[k,g]$, and has the following form:
\begin{equation}
\begin{split}
P_1[k,g] &=\tilde{H}[k,f_s] = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^1_g}\\
P_2[k,g] &=\tilde{H}[k,4f_s] = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^2_g}
\end{split}
\end{equation}

Hence, we can obtain the phase change between 2 groups $\phi^1_{g+1}-\phi^1_{g}, \phi^2_{g+1}-\phi^2_{g}$ due to some contact force applied during this time by taking conjugate multiplication:
\begin{equation}
\begin{split}
\tilde{P}_1[k,g] &= P_1[k,g+1]*\text{conj}(P_1[k,g]) \\
           &= \alpha_s \cancel{e^{-j2\pi k F \frac{d_s}{c}}} e^{j\phi^1_{g+1}} \alpha^{*}_s \cancel{e^{j2\pi k F \frac{d_s}{c}}} e^{-j\phi^1_g+1}\\
           & = |\alpha_s|^2 e^{j(\phi^1_{g+1}-\phi^1_g)}
\end{split}
\end{equation}
Hence, we have
\begin{equation}
\angle{\tilde{P}_1[k,g]} = \phi^1_{g+1}-\phi^1_g, \angle{\tilde{P}_2[k,g]} = \phi^2_{g+1}-\phi^2_g 
\end{equation}
for each subcarrier $k$. We can assume that the required phase change is almost constant with subcarrier index given the low bandwidth, ($f_c+k\Delta F \sim f_c$). This allows us to measure the phase change at multiple subcarriers and finally we can take an average (over subcarrier indices $k$) here to get to one sample value of phase change from either sides of the sensor. Thus by observing $\text{mean}(\angle{\tilde{P}_1[k,g]}), \text{mean}(\angle{\tilde{P}_2[k,g]})$ over multiple phase groups, we can identify the action of a contact force $F$ which acts on the sensor and induces these phase changes.



==> design_v2.tex <==
% !TEX root = main.tex

\section{Design of \paperTitle}

\name consists of a wireless reader that can read the force magnitude and its contact location from the \name sensor. Furthermore, \name's sensor design beyond force magnitude and its contact location, are that it should be robust, low-power, low form-factor, and low complexity, allowing the sensor to be deployed in diverse application scenarios like soft robotics~\cite{}. In this section, we present the design principles of \name. First, we describe \name's force sensor, which translates the force applied and its contact location to change in the properties of RF signal (like amplitude, phase). Next, we present novel algorithms to measure change in the RF properties to deduce the force and the contact location wirelessly. Finally, we conclude with a robust channel measurement technique that uses a wireless waveform to read the sensors while rejecting multi-path.

% force to length
% length to phase
% go about how to measure this phase
% Process: Wireless Reader outside, surfae continuum press on it, detect point+force. This information done 
% while being low power. Sensing/Commn component. Sensing thus is dependent on multipath/SQ/
% Intro like the organization, 

% At heart of WiForce lies  key design components which allow it to sense contact forces wirelessly with low power consumption and minimal electrnics requirement. 
% Fig.~\ref{fig:design_overview} illustrates the design overview of WiForce.
% \todo{you are killing all the surprises in the paper here itself, not going in detail...}
% \todo{this can be background and motivation section, where you explain why you need to make it low power and electronics less, here the requirements and solutions are muddled up and things presents without excitement...}
% \todo{I don't like the writing of this section, it is very non-linear you didn't explain me the phase and how phase can get force and jumped direclt to wireless part}

% At the heart of WiForce lies the key design principle of using minimal electronics to enable sensing with extremely low power consumption. 
% We therefore follow the design principles of backscatter communications, where instead of generating and transmitting the wireless signal, which requires various circuit components like mixer, LNA and high frequency clock sources, WiForce leverages altering the phase of the reflected signals in order to communicate information about contact force. 
% However, wireless signal phase is a very fickle entity, easily corrupted by timing offsets, hardware non-idealities and multipath effects. 
% Hence, as a first step towards building such a passive force sensor, WiForce designs a robust algorithm to isolate sensor's signals from the environmental clutter which allows for accurate wireless phase sensing. 

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Design overview figure here}%
%   \caption{Fig. summarizing the whole design}
%   \label{fig:design_overview}
% \end{figure}


% When interacting with the sensor, the contact locations from either end of the sensor can be linked to contact force by which the sensor is being interacted with.  

% WiForce uses the popular technique of on-off keying modulation of the reflected signal, via a RF-switch to isolate the reflected signal from the LOS signal. 
% Performing two-ended sensing with naive on-off keying modulations, with the requirement of frequency and time isolations, poses issues with inter-modulation and phase discontinuity. 
% To resolve this, WiForce designs a novel clocking strategy which isolates the two ends electrically to reduce inter-modulation, at the same time preserving frequency isolation, which allows reflected phases to be read independently from both the ends of the micro-strip line.

% Finally, equipped with the force sensing micro-strip line prototype and two-ended backscatter solution, WiForce designs a wideband sensing algorithm to isolate the sensor reflected signal from the ambient multipath signals, in order to perform very accurate phase change measurements. 
% WiForce's sensing algorithm borrows elements from Doppler sensing algorithms traditionally used with FMCW/UWB radar system. 
% The key insight here is that the on-off keying gives the sensor an artificial Doppler which can then be sensed via these traditional Doppler sensing algorithms. 
% However, instead of utilizing hardware intensive solutions like FMCW/UWB, we show that equivalent algorithms can work in-general with any wideband channel estimation strategy, and as a demonstration, we showcase this with a simple OFDM based channel estimation method.
% On the other hand, the sensor height plays a more crucial role here, affecting both the force transduction mechanism and RF impedance matching, which requires a careful 
% Force sensing mechanism
% Phases to Forces

% OFDM: Can get in implementation
% S11 figure (Fig. 9) can go in implementation
% Justify the sensor design

\subsection{Force Transduction Mechanism}
\label{subsec:force_transduction}
% First Para: Set up why we would be using microstrip line
As a first step to sense force wirelessly, \paperTitle has to form a connection between the contact forces applied in newtons and its contact location to the measurable properties of RF signals like amplitude and phase. 
The first observation that helps make this connection is that force typically tends to deform/bend physical objects, changing the object's physical dimensions like shape and length. 
Furthermore, these changes can manifest themselves as changes in the RF signal phase, if the RF signals were propagating through the object.
Hence, to design such a wireless force sensor, the strategy would be to choose an object that supports the propagation of RF signals, like transmission lines, and understand how the underlying signal propagation properties would vary due to applying a particular force onto them.
These observations lead \paperTitle to its first design principle, wherein it chooses this physical object undergoing shape deformation as a simple microstrip line. 

% Set up beam bending
A microstrip line consists of two parallel conducting traces, the signal trace, and the ground trace. 
A force applied to the microstrip line causes the traces to bend and come in contact, which shorts the line and leads to signal reflections. This bending phenomena under the action of a force can be explained by viewing the microstrip line traces as mechanical beams and leveraging popular beam-bending models. The reflections produced by the shorting have different phase properties based on the location of the short. \name, therefore, combines concepts from RF microstrip lines and beam mechanics to design a sensor that transduces contact forces into measurable RF phase changes.

% Why naive designs not work
% To enable a force sensitive microstrip line, using just two thin copper sheets as air-separated parallel traces will not be enough. 
% Traditionally, microstrip lines have a dielectric medium filled between the two parallel traces. To allow the deformation in a microstrip line due to forces, the chosen dielectric material has to be deformable and fluid. Amongst the 
However, a naive air-substrate microstrip line will not be force-sensitive at all. For such a design, the beam thickness is infinitesimally low, and irrespective of the contact force applied, the traces will touch each other at virtually a single point (Fig.~\ref{fig:mech_impla}). The contact point invariance leads to a near invariant phase response as force is changed (Fig.~\ref{fig:mech_imple}), therefore preventing the measurement of force through phase changes.

\paperTitle puts a soft beam on top of the signal trace to make the microstrip lines force sensitive. The soft beam follows predictable mechanical models and distributes the force applied along the length of the trace. The distributed force leads to a finite length of the signal trace to come in contact with the ground trace, creating two distinct shorting points, as shown in Fig.~\ref{fig:mech_implb}.Further, these shorting points shift towards the ends as the applied force magnitude increases. Varying shifts induce different phase changes since the signals travel lesser distance on the microstrip line before getting reflected at the shorting points. Hence, the reflections caused by higher magnitude forces accumulate lesser phases relative to the reflected phases when lower force was applied. Thus, the soft beam augmented microstrip line allows us to transduce force to phases (Fig.~\ref{fig:mech_imple}).


\begin{figure}[t!]
\subfloat[Thin traces show saturation of shorting points with increased contact force]{\includegraphics[width=0.49\linewidth]{figures/mech_impla.pdf}\label{fig:mech_impla}}\hfill
\subfloat[Traces with a thick soft layer distribute the forces which allow for more shifting of shorting points]{\includegraphics[width=0.49\linewidth]{figures/mech_implb.pdf}\label{fig:mech_implb}}\\
\vspace{2mm}\\
% \subfloat[Sensor with thin trace]{\includegraphics[width=0.49\linewidth]{figures/mech_implc.pdf}\label{fig:mech_implc}}\hfill
% \subfloat[Sensor with soft layer]{\includegraphics[width=0.49\linewidth]{figures/mech_impld.pdf}\label{fig:mech_impld}}\\
% \vspace{2mm}\\
\subfloat[Due to saturation, thin trace sensors do not show much pronounced phase changes as applied force increases]{\includegraphics[width=1\linewidth]{results/mech_impl_e.pdf}\label{fig:mech_imple}}
\caption{Improving force to phase transduction via aid of soft ecoflex beam}
\label{fig:mech_imp}
\end{figure}


\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/transduction_imga.pdf}
  \caption{Beam Bending: Shorting points shift further apart as the force magnitude increases}
  \label{fig:transductiona}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/transduction_imgb.pdf}
  \caption{Phase Changes due to Beam Bending: Phase-force profiles for the three scenarios above obtained via VNA experiments}
  \label{fig:transductionb}
\end{subfigure}
\caption{The shifting of shorting points due to increased force changes the reflected phase on both the ports, and depending on the location where force is applied both the ports different phase-force profiles.}
\label{fig:transduction}
\end{figure}

% \todo{make location a problem first, then provide solution}
% However, this beam bending effect manifests itself in the form of a varying phase-force relationship depending on the point of application of the contact force (Fig.~\ref{fig:transductionb}). When the contact force is applied at the middle of the sensor, reflected signals from both the ends show similar phase changes since the shorting points move symmetrically. When force is applied towards the ends of the sensor, the part of beam closer to the point of application, shows more phase shift as compared to the other. This is because, the shorter section of the beam is more sensitive to contact forces and bends freely. In comparison, the longer, heavier section essentially collapses onto the bottom trace, which leads to the shorting point being almost stationary as force increases (Fig.~\ref{fig:transduction}). This asymmetric behaviour of phase change with force contact location necessitates sensing of phases from either ends of the sensor. Further, doing so not only enables us to estimate the magnitude of applied force, but also the location it was acting upon. 

However, this beam bending effect manifests itself in the form of a varying phase-force relationship depending on the contact force's point of application (Fig.~\ref{fig:transductiona}). A force applied in the middle of the sensor compresses it symmetrically, and therefore the reflected signals from both the ends show similar phase changes. In contrast, a force that acts asymmetrically will disproportionately compress the smaller length of the beam. Therefore, the end near the smaller length shows a higher phase shift than the end near the longer one. The longer length collapses onto the bottom trace, leading to an almost stationary shorting point as forcing increases (Fig.~\ref{fig:transduction}). This asymmetric behavior of phase change with force contact location necessitates sensing phases from both ends of the sensor. The double-ended measurement allows us to estimate the applied force's magnitude and its location along the sensor length. 

% From the cantilever beam bending models, the beam bends differently if the forces are applied on the ends of the sensor, as compared to forces applied towards the middle of the sensor. In fact, there is a one-to-one relationship between the applied force location and the initial shorting point on the sensor, i.e. 

% % \subsubsection{Contact Force and sensor shorting lengths}
% % 3d, new dimesnion
% A number of past works have used micro-strip lines to create backscatter/RFID based touch sensors to infer touching points along the length of the sensors~\cite{li2016paperid,pradhan2017rio,gao2018livetag}. 
% However, all of these were either printed on a paper, or had a very thin fixed height solid substrate. 
% WiForce adds a new dimension in design of such sensors, by prototyping micro-strip lines with air as substrate, which allows interaction not only along the length, but also height (Fig.~\ref{fig:design_intro}).

% \begin{figure}[h]
%   \centering
%     \includegraphics[width=0.5\textwidth]{figures/design_intro.pdf}
%   \caption{WiForce vs past RFID based touch sensing works: The vertical separation and capability for two-ended sensing allows WiForce to estimate not only the touch location, but also the contact force}
%   \label{fig:design_intro}
% \end{figure}

% This added vertical dimensionality manifests itself as two-ended touch sensing, i.e., due to the vertical air separation between the ground and signal trace, the applied contact force is related to the shorting lengths on either ends. 
% This relationship is governed by traditional mechanical models pertaining to how a cantilever beam deforms under application of a contact force. 
% As the beam starts deforming more and more as the applied force increases, more of the signal trace comes into contact with ground trace, which changes the shorting lengths on either ends. 
% Finally, the reflected signal phase would depend on how much did the signal travel before getting reflected from the shorting point. 
% Hence, ultimately, by sensing phase changes from the either ends of the microstrip line WiForce can sense more than just binary touch, but also the contact force by which the touch interaction occurred.  

% \input{mech_design.tex}

\subsection{How to Sense Force Wirelessly?}
\label{Subsec:double-ended}
As described in the previous section, knowing phase changes from both ends of the sensor allows for measuring and locating the applied force. This section describes the challenges of measuring these phases wirelessly: First, we delineate the method to get a single-ended wireless phase measurement robust to environmental effects. Then we elaborate on the challenges in extending the measurement to both ends and describe our novel switching design that allows it.

% How wired readings are taken
Sensing these phases from either side of the sensor to estimate the force magnitude and location can be done using a wired measurement device like a Vector Network Analyzer (VNA). A VNA typically enables $2$-port analysis of a device-under-test (DUT), i.e., it sends RF signals from both ends of the DUT and measures the reflection properties (amplitude and phase). Therefore, the phase changes due to the shorting points can easily be measured in a wired setup using a VNA.
% Transitioning to wireless challenges
However, wirelessly performing the same task is far from trivial. The wireless signal's phase is easily corrupted by timing offsets, hardware non-idealities, and environmental multipath effects. Further, the concept of obtaining the absolute phase change due is challenging since any wireless phase measurement would also account for the phase accumulated by traveling some distance over the air.
% This challenge is only exacerbated when the signal whose phase we are interested in is a backscattered signal. That is, the signal is not generated at the sensor, but instead is the reflection of an excitation signal sent by the transmitter, undergoing absorption/reflection losses at the sensor and also traveling more distance than the direct path excitation signal. 
% The receiver here has to read the phase of the backscattered signal, under the presence of a much stronger excitation signal. 

% How to isolate signals from the sensor: easy RFID version, and setting up phase problem
% To estimate the phases from the sensor, a first step is to decode the signal coming from the sensor.
% For this, WiForce utilizes the simple power efficient On-Off Keying (OOK) strategy common to RFID systems. OOK basically multiplies the received signal with a square wave of certain frequency, and then transmits it across. 
% This multiplication causes frequency shifts in the reflected signal, and the wireless reader can read the signal at these shifted frequencies to decode the signal from the OOK enabled backscatter device.
% This frequency shift occurs because the square wave can be expanded as fourier series to be decomposed into sinusoidal signals with frequencies as the odd multiple of the fundamental frequency of the square wave.
% Multiplication with sum of these odd frequency sinusoidal tones causes frequency shifts in the reflected signal.
% Since the strategy to decode signals from the sensor has been described, we now address the elephant in the room, i.e. how to estimate these phase changes occurring due to forces being exerted on the sensor.

\begin{figure}[h]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/one_ended_figa.pdf}
  \caption{Before force is applied}
  \label{fig:contactlengtha}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/one_ended_figb.pdf} 
  \caption{After force $F$ is applied}
  \label{fig:contactlengthb}
\end{subfigure}
\caption{Modulation with a square wave (blue) allows isolating the reflected signal from the excitation signal. Observing differential phase ($\angle r_1(t)-\angle r_2(t) = \phi_{\text{full}}+\cancel{\phi_{a}}-\phi_{\text{touch}}-\cancel{\phi_a}$) allows to get rid of phase accumulated over the air (cyan) and gives measure of phase change due to shorting of the microstrip line}
\label{fig:contactlength}
\end{figure}

% Set up differential phase problem
The key idea that allows wireless measurement is the observation that force information is embedded in the differential phase and not the absolute phase. A force applied to the sensor changes the reflected signal's phase, but the phase changes due to air propagation, environmental effects, and hardware offsets remain fixed. Therefore, the differential measurement allows us to bring out only the difference due to the sensor. The difference manifests as a phase jump due to the creation of shorting points on the sensor. By observing the differential phase from both ends of the sensor, one can infer how much contact force caused this phase jump.\\
\noindent \textbf{Sensing differential phase from one end of the sensor:}
% Start with how the sensor signal can be decoded
To estimate the differential phase from the sensor, an initial requirement is to first decode the signal coming from the sensor.
For this, WiForce utilizes RF switches toggling at a particular frequency to modulate the reflected signal, similar to RFID based backscatter systems~\cite{luo20193d,josephson2019rf,freerider}.
The tag receives the excitation signal $s(t)$ and reflects $s(t)m(t)$ where $m(t)$ is a square wave, with time period $T$. Expanding $m(t)$'s Fourier series, we get odd harmonics, $m(t) = \sum_{k\in (2i+1), i\in \mathbb{Z}} \frac{1}{|k|}e^{(j2\pi kf_st)}$ where $f_s=\frac{1}{T}$. 
Ignoring the high order harmonics, we get reflected signal as $r(t) = s(t)m(t) \approx s(t)e^{j2\pi f_s t}$. 
Hence the reflected signal will be shifted by frequency $f_s$, which allows the reflected signal, $r(t)$, to be isolated from the excitation signal, $s(t)$ in the frequency domain. 

Hence, to sense differential phase from the sensor, the wireless reader reads the phases at shifted frequencies, and observes the phase jumps caused by the shifting of contact edges between the traces due to an applied force (Fig.~\ref{fig:contactlength}). 
Denote the reflected signal just before/after a contact force was applied as $r_1(t)/r_2(t)$. From, Fig.~\ref{fig:contactlength} $\angle r_1(t) = \phi_{\text{full}}+\phi_a$, from the wireless propagation over the air and over the entire length of the sensor. Similarly, $\angle r_2(t) = \phi_{\text{short}}+\phi_a$, since now the signal got reflected back from the shorting point. 
Thus, the differential phase between $r_1(t), r_2(t)$ would be $\phi_{\text{full}}+\cancel{\phi_{a}}-\phi_{\text{short}}-\cancel{\phi_a}$, and thus the differential phase jump would give us $\phi_{\text{full}}-\phi_{\text{short}}$. Since $\phi_{\text{full}}$ is the net phase accumulated by the signals by traveling the full length of the microstrip line, this is a fixed quantity that can be calibrated beforehand from accurate VNA readings. Thus, reading the differential phase allows us to estimate  $\phi_{\text{full}}-\phi_{\text{short}}$, and in turn, $\phi_{\text{short}}$, which is the phase due to the shifting of contact points caused by an applied force. 

% Why naiveity wont work
\noindent \textbf{Sensing differential phase from both the ends of the sensor:} A naive extension to the single ended measurement is to have RF switches on both ends of the sensor, toggle them at different frequencies ($f_{s_1}/f_{s_2}$), and read the phase jumps at these shifted frequencies. Although this solution to sense phase jumps from both ends is correct in spirit, there is more to the double-ended sensing problem than just simple frequency multiplexing. To estimate the differential phase, it is required to sense the phase before force was applied, in which the sensor acts like a perfectly conducting microstrip line between the two ends. In this scenario, if both the switches are toggled-on, the signals will propagate through the sensor and leak out from the other end. This causes intermodulated reflections, where the reflected signal would be partially modulated by both toggling frequencies. This is visually illustrated in Fig.~\ref{fig:intermod}.

\begin{figure}[!t]
\centering
\includegraphics[width=0.45\textwidth]{figures/intermod.pdf}
\caption{Different freq. clocks introduce intermodulation due to both switches being toggled on (red shaded time instants)}
\label{fig:intermod}
\end{figure}

% Hence, the question to be posed is, how to avoid this intermodulation issue? When one switch is toggled-on to connect to the sensor, the other switch has to be toggled-off to act like an open reflector\footnote{The design setup hence requires reflective RF switches}, in order to avoid the intermodulation outputs.
The challenge in avoiding the intermodulation effects is that the sensor has to reflect signals from the opposite end when a switch is toggled on. Using reflective RF switches in the off state allows us to make either of the ends reflective, under the restriction that the other should be off when one switch is on.
\if 0
 By observing this, a naive attempt would be to consider time multiplexing instead. That is, at a given time only one switch toggles and the other is terminated, and after a definite time slot the roles reverse. However, this would then complicate the differential phase algorithm since it would be required to track the phase jumps arising due to clocks turning on and off. Further, it would limit the potential usage of multiple such sensors in tandem, since this time scheduling has to be agreed upon over multiple of these sensors. To bypass these issues, WiForce presents a unique clock design which would avoid the intermodulation issue and at the same time provide frequency separation for the reflected signals coming from either end.
\fi
The unique insight which allows WiForce to have such a on-off scheme is the use of duty cycle properties of square wave Fourier series. In a standard square wave, with $50\%$ duty cycle, all the even harmonics (i.e. every second harmonic) are absent. Similarly, in a wave with $25\%$ duty cycle, every fourth harmonic would be absent. Hence, a frequency $f_s$, $25\%$ duty cycle square wave will give modulation at $\underline{\mathbf{f_s}},2f_s,3f_s,\cancel{4f_s} 5f_s, \ldots$  Similarly, a frequency $2f_s$, $25\%$ duty cycle square wave will give modulation at $2f_s,\underline{\mathbf{4f_s}},6f_s,\cancel{8f_s},10f_s\ldots$ Observe that a combination of these 2 clocks will cause interference at $2f_s$, but can be read up individually at $f_s$ for the former clock, and $4f_s$ for the latter clock. Hence, a combination of these 2 clocks can provide separation in the frequency domain. Also, by controlling the initial phases of these two clocks, we can suppress the intermodulation problem as well. This is possible because when one clock is high, the other clock will be guaranteed to be low and vice versa (Fig.~\ref{fig:two-sided}). Hence, at any given time, only one port will be on, and other port will be reflective open. Further, to reduce the form factor requirements, instead of having $2$ antennas, one for each end of the sensor, we can just have just a one antenna design using a splitter. Since the clocking strategy provides separation in the frequency domain, we can add the modulated signals from the either ends via a splitter. Thus, we can read the differential phases at $f_s, 4f_s$ due to new shorting points caused by the bending of the sensor under an applied force $F$.
\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{figures/two-ended.pdf}
\caption{The two-ended sensing approach of WiForce. At any time instant, only one switch is toggled on}
\label{fig:two-sided}
\end{figure}

\subsection{Rejecting Multipath by Reading Forces at Multiple Frequencies}
\label{Subsec:wideband}

% By utilizing the clock design strategy discussed, phases from both ends of the sensor are modulated with different shifted frequencies, which distinguish them from the excitation signal which is received directly without any frequency shifts. 
In this section, we describe how \name uses general wideband channel estimates to measure differential phase across both ends of the sensor. The key insight of WiForce here is that periodic wideband channel estimates can be utilized to detect the frequency shifts coming from the sensor modulations. Further, going one step ahead, we can even harness tremendous averaging gains by reading the same differential phase over the entire channel estimation bandwidth.
% In contrast, most of the past phase sensing solutions for RFID based touch sensing have largely used narrowband sensing, which further require a specialized RFID reader~\cite{pradhan2017rio}, whereas WiForce's solution can work with commodity 
% Thus, WiForce first comes up with a strategy to sense these phases from periodic channel estimates. 
Therefore, \name's strategy becomes waveform-agnostic, and can be used with any wideband sensing waveform that allows for periodic channel estimates, such as FMCW, UWB and OFDM.

WiForce's strategy consists of two steps: 
The first step involves viewing the frequency shift originating from square wave modulation as an `artificial-Doppler', since Doppler effects also introduce similar frequency shifts.
\name utilizes an FFT-based technique of sensing these frequency shifts, which works very similar to how Doppler is traditionally sensed via wideband sensing waveforms like FMCW and UWB~\cite{josephson2019rf}. We show that this algorithm works with a lower bandwidth (12.5 Mhz) OFDM based channel sounding approach. Since force information is in the form of phase changes unaffected by environmental effects and air propagation, we do not need absolute time-of-flight measurements, avoiding very high bandwidth (100s of MHz) typical of FMCW/UWB. 

\if 0
\notdone{\%\% The next few lines motivate the sensing strategy can be used in intro as well, just writing it here to put these thoughts into words \%\%}
Also, making the sensor design work with OFDM-based channel sounding provides interesting opportunities for communication and sensing to co-exist and allows for seamless future integration with Wi-Fi-based solutions. Further, in doing so we introduce a paradigm shift in backscatter sensing solutions, wherein, we don't require the quantization of data into bits and the sending of them over a low throughput link, but the data is instead embedded in the phase differences in channel estimates, and can be read continuously at the receiver. The former strategy requires presence of low power ADCs/data buffers to quantize and communicate the data, in addition to RF switches to isolate the reflected signal from excitation signal, whereas our solution just requires RF switches toggling with a certain clocking strategy. To justify the usage of these ADCs/data buffers, the former strategy requires presence of an explicit wake-up signal so that these power hungry components are used only for a fraction of time. In comparison, our design does not require the presence of such wake-up signals and can be turned-on all the time. Hence, we believe this sensing paradigm would pave the way forward to ultra low-power backscatter sensing links, which can work even in challenging environments like inside body tissue, where the efficiency of RF harvesters might not be able to support the sensing paradigms requiring ADCs/data buffers. \notdone{\%\% End of sensing motivation block\%\%}
\fi 
% Hence, now we will present how WiForce uses OFDM channel sounding to read the phase changes coming from either end of the sensor. 
\begin{figure*}[h]
\centering
\includegraphics[width=0.95\textwidth]{figures/ofdm_expl.pdf}
\caption{WiForce's sensing algorithm which utilizes wideband channel estimates to isolate the signal from multipath in Doppler domain. Finally, by grouping the channel estimates into `phasegroups', WiForce can read phase changes over multiple subcarriers which allows for averaging gains to make the phase sensing robust and accurate}
\label{fig:ofdm_expl}
\end{figure*}

The algorithm to estimate the two-ended differential phase embedded inside the wideband channel estimates is visually illustrated in Fig.~\ref{fig:ofdm_expl}. Say we are estimating the channel periodically after every $T$ seconds, with frequency steps of $F$ (this could be subcarrier spacing/sweep step in OFDM/FMCW based waveforms). We denote $H(kF,nT) = H[k,n]$ where $k$ is subcarrier index and $n$ is time index. Now, if there are $M$ multipaths in addition to the signal coming from the sensor, we can write the channel estimates as $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + (s_1(nT) e^{-j\phi^1_n} +s_2(nT)e^{-j\phi^2_n})\alpha_s e^{-j2\pi k F \frac{d_s}{c}}$

Here, $\alpha_i$ is the attenuation factor for the $i$-th path, $d_i$ is the distance separation between the TX-reflector and reflector-RX, and $\phi^1_n, \phi^2_n$ is the phase accumulated from the RF propagation in the microstrip line sensor at time index $n$ from sensor end $1$ and sensor end $2$. $s_1(t),s_2(t)$ are the double-ended sensor modulation as per the duty cycled clocking strategy discussed earlier. Expanding them as harmonics, we get $s_1(t) = \sum_{p\neq 4q, q\in \mathbb{Z}} a_p e^{j2\pi pf_{s_1}t}$, $s_2(t) = \sum_{p\neq 4q, q\in \mathbb{Z}} a_p e^{j2\pi pf_{s_2}t}$. We have $f_{s} = f_{s_1} = 0.5f_{s_2}$ and thus modulations at $f_{s}, 4f_{s}$. Ignoring the higher harmonics and the constant factors $a_p$ associated with the Fourier expansion for brevity, we get $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})$
% \begin{equation}
% \resizebox{0.45\textwidth}{!} 
% {
%     $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})$
% }
% \end{equation}
% \begin{equation}
% \begin{split}
%  H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} +&  \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+\\ &e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})
%  \end{split}
% \end{equation}

Now, to isolate the signal coming from the sensor, we take FFT over the $n$-th index, to obtain $\tilde{H}[k,f]$. We observe $N$ channel snapshots and take the following transform:
\begin{equation}
\tilde{H}[k,f] = \sum_{n=1}^N H[k,n] e^{-j2\pi f n T}
\end{equation}

Observe that for this transform, the nyquist frequency would be $\frac{1}{2T}$, and hence, $f_s$ has to be chosen such that $4f_s \leq \frac{1}{2T}$. Hence, assuming $\phi^1_n, \phi^2_n$ stay constant over the period of $N$ snapshots, at $f_s$, $4f_s$, we have,
\begin{equation}
\begin{split}
\tilde{H}[k,f_s] &= \sum_{n=1}^N H[k,n] e^{-j2\pi f_s n T} = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^1_n}\\
\tilde{H}[k,4f_s] &= \sum_{n=1}^N H[k,n] e^{-j2\pi 4f_s n T} = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^2_n}\\
\end{split}
\label{eqn:sensharmonics}
\end{equation}

This draws a parallel to how Doppler is sensed from wideband sensing algorithms, and switching in fact gives the sensor an `artificial Doppler' which can be sensed as done above. The switching frequency $f_s$ can be related to an equivalent Doppler, $f_s = \frac{f_c v}{c}$, and thus an object in the environment moving at velocity $v = \frac{c f_s}{f_c}$ would create interference with the sensor signal. However, the chosen $f_s$ is large enough so that this equivalent speed is so high that it wouldn't appear in the environment for the use cases considered. Hence, taking this FFT isolates the signal coming from the sensor and nulls out the multipath clutter in the environment. 

Recall that while writing Eqn.~\eqref{eqn:sensharmonics}, we assumed $\phi^1_n, \phi^2_n$ stay constant over the period of $N$ snapshots. Basically, this assumes that the force acting on the sensor stays almost constant for about $N$ snapshots, which is a reasonable assumption given it requires some time for mechanical beams to relax and get to steady state under the action of force. Said differently, wireless sensing occurs at much higher sampling rate (about order of MHz), whereas the mechanical forces are much slower (take about 0.5-1 seconds to stabilize). 

Thus, WiForce designs an algorithm to sense these phase differences from the filtered harmonics, and ultimately map them to applied force. The algorithm divides the channel estimates into groups of $N$, referred to as `phase-groups'. For each phase-group we first take the harmonics FFT as described earlier and obtain $2$ $K\times1$ vector from Eqn.\ref{eqn:sensharmonics} for FFT frequency $f_s$, $4f_s$. Assuming there are $N_g$ such phase groups, and for all $N$ samples of $g$-th group, $\phi^1_n,\phi^2_n \approx \phi^1_g \phi^2_g \forall n \in \{1,2,\ldots N\}$. The output at $g$-th phase group, $k$-th subcarrier, after harmonics FFT at $f_s, 4f_s$, is denoted as $P_1[k,g],P_2[k,g]$, and has the following form:
\begin{equation}
\begin{split}
P_1[k,g] &=\tilde{H}[k,f_s] = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^1_g}\\
P_2[k,g] &=\tilde{H}[k,4f_s] = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^2_g}
\end{split}
\end{equation}

Hence, we can obtain the phase change between 2 groups $\phi^1_{g+1}-\phi^1_{g}, \phi^2_{g+1}-\phi^2_{g}$ due to some contact force applied during this time by taking conjugate multiplication:
\begin{equation}
\begin{split}
\tilde{P}_1[k,g] &= P_1[k,g+1]*\text{conj}(P_1[k,g]) \\
           &= \alpha_s \cancel{e^{-j2\pi k F \frac{d_s}{c}}} e^{j\phi^1_{g+1}} \alpha^{*}_s \cancel{e^{j2\pi k F \frac{d_s}{c}}} e^{-j\phi^1_g+1}\\
           & = |\alpha_s|^2 e^{j(\phi^1_{g+1}-\phi^1_g)}
\end{split}
\end{equation}
Hence, we have
\begin{equation}
\angle{\tilde{P}_1[k,g]} = \phi^1_{g+1}-\phi^1_g, \angle{\tilde{P}_2[k,g]} = \phi^2_{g+1}-\phi^2_g 
\end{equation}
for each subcarrier $k$. We can assume that the required phase change is almost constant with subcarrier index given the low bandwidth, ($f_c+k\Delta F \sim f_c$). This allows us to measure the phase change at multiple subcarriers and finally we can take an average (over subcarrier indices $k$) here to get to one sample value of phase change from either sides of the sensor. Thus by observing $\text{mean}(\angle{\tilde{P}_1[k,g]}), \text{mean}(\angle{\tilde{P}_2[k,g]})$ over multiple phase groups, we can identify the action of a contact force $F$ which acts on the sensor and induces these phase changes.



==> intro-v1.tex <==
% !TEX root = main.tex
% From a larger persdpective where the problem stands and what people have tried
% one paragraph one message
% Dont put multiple messages 

\section{Introduction}

Contact force is a fundamental sensing measure that affects how we touch and interact with things around us. Human beings sense this contact force via their skin, which is an extremely sensitive layer, and allows to sense the magnitude and contact location of even a slightest of nudge \cite{}. However, in most of our interactions with digital world, mostly via our smartphones, laptops and tablets, the sense of force is replaced with a simple sense of touch (contact or no contact), i.e. we mostly interact with these entities just by our sense of touch with these devices completely oblivious to how much force is applied. \margins{fixed -- this is a bit unclear... what is meant by a ``naive sense of touch"?} In the next generation of user-interactions, with upcoming VR interfaces, interactions with different objects would require necessitate contact force in addition to touch. Apple and Google have already started exploring force feedback for richer UI experience \cite{quinn2019estimating}, and latest iPhones and Apple watches come equipped with a capacitative force sensor \cite{Apple3Dtouch} to provide haptic feedback to the user. 



\begin{figure}[H]
  \centering
    % \placeholder[width=0.3\textwidth]{$l_1,l_2$ figure here}%
    \includegraphics[width=0.5\textwidth]{figures/appl.pdf}
  \caption{Applications targeted by \paperTitle: Interactions with different solid objects via VR interfaces will require more than just touch feedback. Surgical robots inside the body inadvertently touch other tissues, leading to potential risks. Finally, force sensitive robotic grippers could open up new automation possibilties.}
  \label{fig:appl}
\end{figure}

\margins{Text on the surgical robot subfigure is much too small. Also what is the circle at the tip of the robot, and the yellow and blue lines? I'm not sure what is meant in the caption by ``more than just touch feedback". Also, if you are pitching interaction with solid objects, then the statue in the VR subfigure should not be transparent?}

Ability to sense the applied contact force ubiquitously on a surface, could similarly open up a lot of interesting possibilities and add a new dimension to the sensing capabilities of these upcoming smart surfaces. 

However, our force sensing modalities have to be upgraded significantly to allow for continuum force sensing. 
Further, this sensing lacuna has inhibited the advancement of robotic manipulators, entities which try and mimic human hands, since they have no sense of haptic feedback which human hands are so sensitive against. This severely limits the application capabilities of these robots, to an extent that one of the main roadblock to enabling these precise robotic surgeries is that doctors can't ascertain if the path taken by the robot is safe or not \cite{alemzadeh2016adverse}. That is, doctors do not know if while operating on a certain tissue the robot is applying a contact force that is appreciably large to hurt the tissue. Hence, there has to be a feedback in terms of continuum contact force sensing to help the doctors in identifying safe operation of the surgical robot inside the human body.

Thus, force sensing has garnered a lot of research interest across various communities, like surgical robotics \cite{tegin2005tactile,trejos2010force}, Human-Computer interaction (HCI) \cite{quinn2019estimating,boceck2019force}, and prosthetics research \cite{merrett2010augmenting}. Force sensing has even been posed as a `Grand Challenge' for further advancement of surgical robotics \cite{burgner2015continuum}. Typically force sensing has been attempted with sensing principles like strain gauges, load cells, FBG based optical fibres and force sleeves. Each of these sensing principles sense force only at discrete mounting points, and not across the entire surface/length of the sensor. This limits the usage of these sensors and thus these sensors can not create a rich continuum sensing experience offered by our skin which we are typically used to.
% Worse, not one of these sensing principles is universally optimal. Depending on whether you would want to sense force at the tip, or near the robot-tissue interface, the appropriate choices are strain gauges and force sleeves respectively. 
Hence, there is a need for a sensing principle which can sense force across the surface, and the main goal here should be that the sensing principle should, in effect act like a continuum artificial skin, instead of providing force measurements at discrete points.

% Robotic manipulators hold a huge potential in surgery robotics, where they can go beyond mimicking a human hand and perform far more intricate surgeries than possible by a human hand. However, unlike a human hand, these robotic manipulators are completely oblivious to the magnitude of force they touch their environment with.  Hence, there has to be a feedback in terms of continuum contact force sensing to help the doctors in identifying safe operation of the surgical robot inside the human body.

% Sensing touch interactions on surfaces has also attracted a lot of research interest in the wireless sensing community \cite{pradhan2017rio,li2016paperid,gao2018livetag}. The systems have demonstrated detection of gestures/swipes alongside simple touch events on passive surfaces, which have a lot of HCI applications of extending UIs to such passive surfaces. However, these works are limited in the sense that these can't distinguish events wherein a person is touching with higher/lower force, and in a way provide just 1 bit information related to the touch event. 

\paperTitle presents design, implementation and evaluation of a sensor prototype which can sense force throughout the sensor surface and thus address the continuum sensing lacuna with the current force sensors. The two broad themes which \paperTitle's sensor design targets are providing haptic feedback for surgical robots, and a smart force sensitive passive surface design. Fitting to the two broad themes, the sensor transduction mechanism is coupled with an extremely low power backscatter link, for wireless force feedback to enable safe battery-free operation of surgical robots inside the body, and creation of passive force sensitive surfaces. 

Hence, instead of generating wireless signals, \paperTitle conveys the force information by changing the phase of reflected signals. A key question which \paperTitle answers is, how can contact force, which is a purely mechanical parameter, be linked to RF signal phase. \paperTitle does this by combining RF and mechanical viewpoint of a simple beam model, consisting of two parallel traces, one being ground trace and other being the signal trace, separated by air. 

\begin{figure}[H]
  \centering
    % \placeholder[width=0.3\textwidth]{$l_1,l_2$ figure here}%
    \includegraphics[width=0.5\textwidth]{figures/bending.pdf}
  \caption{Sensor prototype \& force transduction mechanism}
  \label{fig:intro_fig}
\end{figure}

In RF viewpoint, this is basically a microstrip transmission line with air as substrate, whereas in a mechanical viewpoint this is basically a cantilever beam model. Viewing the sensor as a cantilever beam model allows mapping forces to contact lengths $l_1$, $l_2$ (Fig. \ref{fig:intro_fig}). Viewing the sensor as a microstrip transmission line allows us to map reflected signal phases to the contact locations where the transmission line gets shorted from either ends ($l_1, l_2$, Fig. \ref{fig:intro_fig}). Hence, by forming this connection between RF and mechanical viewpoints, \paperTitle is able to estimate contact force by observing the phase changes due to shorting of transmission line at different locations. 

Further, \paperTitle designs a novel algorithm to detect this phase change accurate to about a degree, which leads to a force resolution of about 0.2 N. The algorithm takes inspiration from how FMCW/UWB systems estimate signal doppler variations, and uses this idea to give an artificial doppler to the sensor by making it switch at certain frequencies. The artificial doppler generated is high enough to make it isolated from any low doppler environmental signals. 
This allows \paperTitle to estimate phase changes super accurately and robust even to dynamic multipath interference, and then map it back to contact force using the cantilever beam model.
However, instead of testing the algorithm with specialized waveforms and ultra-high bandwidths, we show the algorithm working for OFDM based channel estimation to motivate seamless fusion of communication and sensing for this sensing paradigm.

Hence the technical contributions of this paper are
\begin{itemize}
  \item Ideation and fabrication of a novel force sensing paradigm involving transmission lines 
  \item The sensor design is the first one to sense force position and location across the length of the robot
  \item Performing double sided phase measurements from 2 antennas, and a novel algorithm to address the intermodulated harmonics
  \item Performing accurate sensing of phase by isolating reflected signal from the sensor and combating multipath
\end{itemize}


% \paperTitle hence   in force sensing for surgical robots. The sensor can, in principle, sense as well as locate contact force across the robot body. This is achieved by abstracting the sensor as a transmission line model. A transmission line model is generated by viewing the sensor as a lumped model of continuous impedences, to provide data in a continuum fashion. The signal trace of the transmission line can be wrapped across the robotic manipulator, and ground layer being the inner diameter of the robot.This, in-effect act like an artificial skin for the robot. However, given the size limitations and the flexibility requirements, it is imperative that this sensor should provide wireless reading capabilities. 

% We leverage 2 key insights here, which allows us to create such an artificial skin capable of sensing force across the length. Firstly, by using mechanical models like cantilever beams etc, the force measure can be inferred by estimating the contact length of the flexible outer layer of skin, which has the signal trace of the transmission line, with the robotic surface acting as a ground layer. To estimate this contact length, we measure the contact lengths from the either end of the transmission line. This is done by measuring the phase change in the signal due to this pressing motion, as the signal now travels a lesser length before reflecting back. The second key insight we have here is that, since all the force information is encoded in the phase change of the signal, this sensing modality can be readily integrated with wireless sensing paradigms, which also leverage sensor data information encoded in phase of the signal. To do so, we have antennas on either ends of the transmission line, and we perform wireless measurements of phase change induced onto either end of the transmission line, in order to estimate the force location and force magnitude. For this, we address issues like intermodulation harmonics, clock drift and multipath correction, to estimate the phase changes accurately and precisely.

% Hence the technical contributions of this paper are
% \begin{itemize}
%   \item Ideation and fabrication of a novel force sensing paradigm involving transmission lines 
%   \item The sensor design is the first one to sense force position and location across the length of the robot
%   \item Performing double sided phase measurements from 2 antennas, and a novel algorithm to address the intermodulated harmonics
%   \item Performing accurate sensing of phase by eliminating clock drifts and cancelling multipath
% \end{itemize}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/sensor.pdf}
% \caption{Transmission line (yellow) is wrapped around the robot body and acts like an artificial skin layer. The contact force manifests as phase changes $\phi_1$,$\phi_2$ as the transmission line which was previously open ended is now shorted at two contact points}
% \end{figure}


==> mech_design.tex <==
% !TEX root = main.tex




% \notdone{\%\%Very briefly tell how the force gets linked to $l_1$,$l_2$, via simulations (Just show the 3-d plot of F vs $l_1$, $l_2$\%\%}

% % In order to convert the effects of contact forces on the sensor to phase change observed on the microstrip line, \paperTitle is equipped with a beam composed of two layers, fixed at both ends: a rigid one at the top, and a soft one at the bottom. A microstrip line is attached at the bottom of the soft layer. Upon application of a contact force on the beam, the signal trace of the microstrip line bends and comes into contact with the ground trace, located on a fixed, planar beam. The role of each layer is as follows:

% \begin{figure}[H]
%   \centering
%     \placeholder[width=0.3\textwidth]{Can we have a figure with the current model and the simulated model to justify things?}
%     \caption{Phase to Force mapping model}
%     \label{fig:sensor_design_parameters}
% \end{figure}


% Beam mechanics is then used to calculate the maximum displacement of the beam $y_{max}$, as well as its location along the beam, given by Eq.~\eqref{eq:maximum_displacement_value}:
% \begin{equation}
% y_{max} =
% \left\{
% \begin{array}{lll}
% \dfrac{2F_M F_l^2(L-F_L)^3}{3K(3L-2F_L)^2} \!&\! \text{at} \!\quad\! x = \dfrac{L^2}{3L - 2F_L} \!&\! \text{if} \!\quad\! F_L \leq \dfrac{L}{2}\\
% \dfrac{2F_M F_L^3(L-F_L)^2}{3K(L+2F_L)^2} \!&\! \text{at} \!\quad\! x = \dfrac{2 L F_L}{L + 2F_L} \!&\! \text{if} \!\quad\! F_L \geq \dfrac{L}{2}
% \end{array}
% \right.
% \label{eq:maximum_displacement_value}
% \end{equation}
% The contact between the top bending beam and the rigid bottom beam thus occurs for $y_{max} = d$. As visible in Eq.~\eqref{eq:maximum_displacement_value}, the location of the maximum deflection, and thus the contact location between the traces for $y_{max} = d$, is a function the force location $F_L$ only, and creates a unique relationship between force location and contact location between the traces.

% %As the contact force increases, the contact lengths increases since more of the signal trace comes into contact with the ground trace. Hence, by sensing the contact length, we can infer the applied force. This forms the key sensing modality which allows \paperTitle to sense contact forces.

% %However, the relationship between contact length and applied force also depends on where the force is applied along the length of the sensor. Contact length varies differently if the force is applied at the middle of the sensor as compared to towards the ends of the sensor. Hence, it is imperative to sense not only the contact length, but also the exact contact points in order to sense force. 

% A layer of soft, hyperelastic material is added under the beam. It allows, after initial contact between the beams, to convert the applied force to a contact length, creating a unique mapping between force magnitude and the edges of the contact length. The material selected is Ecoflex 00-30, selected for its softness, allowing increased contact area. The variations of contact edges, and thus phase change, based on variations of force magnitude and location, are observed experimentally.



% \textcolor{magenta}{\%\%\%\%\%  \%\%\%\%\%}

% \label{section:sim_comsol}

==> mech_impl.tex <==
% !TEX root = main.tex



%\begin{figure}[t!]
%\begin{subfigure}[t]{.24\textwidth}
%  \centering
  % include first image
%  \includegraphics[width=0.95\linewidth]{figures/mech_impla.pdf}
%  \caption{Thin traces show saturate with increased contact force}
%  \label{fig:mech_impla}
%\end{subfigure}%
% \hspace{0.5em}% Space between image A and B
%\begin{subfigure}[t]{.24\textwidth}
%  \centering
  % include second image
%  \includegraphics[width=0.95\linewidth]{figures/mech_implb.pdf}
%  \caption{Traces with a thick soft layer distribute the forces which allow for finer bending}
%  \label{fig:mech_implb}
%\end{subfigure}

%\begin{subfigure}[t]{.24\textwidth}
%  \centering
  % include first image
%  \includegraphics[width=0.95\linewidth]{figures/mech_implc.pdf}
%  \caption{Sensor prototype with thin trace}
%  \label{fig:mech_implc}
%\end{subfigure}%
%\begin{subfigure}[t]{.24\textwidth}
%  \centering
  % include second image
%  \includegraphics[width=0.95\linewidth]{figures/mech_impld.pdf}
%  \caption{Sensor prototype with Ecoflex soft layer}
%  \label{fig:mech_impld}
%\end{subfigure}
%\begin{subfigure}[t]{.48\textwidth}
%  \centering
  % include second image
%  \includegraphics[width=0.95\linewidth]{results/mech_impl_e.pdf}
%  \caption{Due to saturation, thin trace sensors do not show much pronounced phase changes as applied force increases \notdone{\%\% Artificial plot, To be Generated \$\$}}
%  \label{fig:mech_imple}
%\end{subfigure}
%\caption{Improving force to phase transduction via aid of soft ecoflex beam}
%\label{fig:mech_imp}
%\end{figure}

% \notdone{\%\%Aim: Discuss about soft layer fabrication briefly\%\%}
% To enable a force sensitive microstrip line, using just two thin sheets as air-separated parallel traces will not be enough. 
% This is because for such a naive design, the shorting points will saturate with application of small forces as the beam thickness is very low (Fig.~\ref{fig:mech_impla}).

% To prevent this saturation, \paperTitle has a soft beam on top of the copper trace to allow the force to be distributed evenly across the length of the beam in order for it to follow the beam bending transduction mechanism discussed in Section~\ref{section:force_transduction}. We use Ecoflex to fabricate the soft-layer for our sensor prototype (Fig. \ref{fig:mech_impld}). To confirm the effectiveness of the soft layer design, we fabricate a similar sensor without the soft layer, and map the phases with force. We can clearly see that the naive sensor design doesn't show significant phase change as force increases, since it saturates very early on. However, with the soft beam we get very appreciable phase changes which allow us to use the force transduction mechanism to map phases to contact force (see Fig.~\ref{fig:mech_imple}).

% \begin{figure}[h]
%   \centering
%     \placeholder[width=0.3\textwidth]{Image of the sensor with soft layer}
%     \caption{\paperTitle's sensor prototype}
%     \label{fig:sensor_fin}
% \end{figure}


==> mech_related.tex <==
% !TEX root = main.tex

\noindent \notdone{\%\%Aim: To describe the other sensing modalities/suboptimalities of current force sensing solutions \%\%}


\textbf{Force sensing transductions}: 

There are vareity of way to meausre the force using the load cells, etx... Why are those not good ways of doing continumm force sensing... 


\textbf{Applications of force sensing transductions}: 
\todo{talk about application we can enable using wireless force sensor, which before we couldn't enable}

There are vareity of way to meausre the force using the load cells, etx... Why are those not good ways of doing continumm force sensing... 


==> old_design.tex <==
\subsection{How to Sense Forces Wirelessly?}
\label{Subsec:double-ended}
As described in the previous section, knowing phase changes from both ends of the sensor allows for measuring and locating the applied force. This section describes the challenges of measuring these phases wirelessly: First, we delineate the method to get a single-ended wireless phase measurement robust to environmental effects. Then we elaborate on the challenges in extending the measurement to both ends and describe our novel switching design that allows it.

% How wired readings are taken
Sensing these phases from either side of the sensor to estimate the force magnitude and location can be done using a wired measurement device like a Vector Network Analyzer (VNA). A VNA typically enables $2$-port analysis of a device-under-test (DUT), i.e., it sends RF signals from both ends of the DUT and measures the reflection properties (amplitude and phase). Therefore, the phase changes due to the shorting points can easily be measured in a wired setup using a VNA.
% Transitioning to wireless challenges
However, wirelessly performing the same task is far from trivial. The wireless signal's phase is easily corrupted by timing offsets, hardware non-idealities, and environmental multipath effects~\cite{tse2005fundamentals}. Further, the concept of obtaining the absolute phase change due is challenging since any wireless phase measurement would also account for the phase accumulated by traveling some distance over the air.
% This challenge is only exacerbated when the signal whose phase we are interested in is a backscattered signal. That is, the signal is not generated at the sensor, but instead is the reflection of an excitation signal sent by the transmitter, undergoing absorption/reflection losses at the sensor and also traveling more distance than the direct path excitation signal. 
% The receiver here has to read the phase of the backscattered signal, under the presence of a much stronger excitation signal. 

% How to isolate signals from the sensor: easy RFID version, and setting up phase problem
% To estimate the phases from the sensor, a first step is to decode the signal coming from the sensor.
% For this, \paperTitle utilizes the simple power efficient On-Off Keying (OOK) strategy common to RFID systems. OOK basically multiplies the received signal with a square wave of certain frequency, and then transmits it across. 
% This multiplication causes frequency shifts in the reflected signal, and the wireless reader can read the signal at these shifted frequencies to decode the signal from the OOK enabled backscatter device.
% This frequency shift occurs because the square wave can be expanded as fourier series to be decomposed into sinusoidal signals with frequencies as the odd multiple of the fundamental frequency of the square wave.
% Multiplication with sum of these odd frequency sinusoidal tones causes frequency shifts in the reflected signal.
% Since the strategy to decode signals from the sensor has been described, we now address the elephant in the room, i.e. how to estimate these phase changes occurring due to forces being exerted on the sensor.

% Set up differential phase problem
The key idea that allows wireless measurement is the observation that force information is embedded in the differential phase and not the absolute phase. A force applied to the sensor changes the reflected signal's phase, but the phase changes due to air propagation, environmental effects, and hardware offsets remain fixed. Therefore, the differential measurement allows us to bring out only the difference due to the sensor. The difference manifests as a phase jump due to the creation of shorting points on the sensor. By observing the differential phase from both ends of the sensor, one can infer how much contact force caused this phase jump.\\
\noindent \textbf{Sensing differential phase from one end of the sensor:}
% Start with how the sensor signal can be decoded
To estimate the differential phase from the sensor, an initial requirement is to first decode the signal coming from the sensor.
For this, \paperTitle utilizes RF switches toggling at a particular frequency to modulate the reflected signal, similar to RFID based backscatter systems~\cite{luo20193d,josephson2019rf,freerider}.
The tag receives the excitation signal $s(t)$ and reflects $s(t)m(t)$ where $m(t)$ is a square wave, with time period $T$. Expanding $m(t)$'s Fourier series, we get odd harmonics, $m(t) = \sum_{k\in (2i+1), i\in \mathbb{Z}} \frac{1}{|k|}e^{(j2\pi kf_st)}$ where $f_s=\frac{1}{T}$. 
Ignoring the high order harmonics, we get reflected signal as $r(t) = s(t)m(t) \approx s(t)e^{j2\pi f_s t}$. 
Hence the reflected signal will be shifted by frequency $f_s$, which allows the reflected signal, $r(t)$, to be isolated from the excitation signal, $s(t)$ in the frequency domain. 

\begin{figure}[t!]
\begin{subfigure}{\linewidth}
  \centering
  % include first image
  \includegraphics[width=\linewidth]{figures/one_edned_figa.pdf}
  \caption{Before force $F$ is applied}
  \label{fig:contactlengtha}
\end{subfigure}
\begin{subfigure}{\linewidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{figures/one_edned_figb.pdf} 
  \caption{After force $F$ is applied}
  \label{fig:contactlengthb}
\end{subfigure}
\caption{Modulation with a square wave (blue) allows isolating the reflected signal from excitation signal. Observing differential phase ($\angle r_1(t)-\angle r_2(t) = \phi_{\text{full}}+\cancel{\phi_{a}}-\phi_{\text{touch}}-\cancel{\phi_a}$) allows to get rid of phase accumulated over the air (cyan) and gives measure of phase change due to shorting of microstrip line}
\label{fig:contactlength}
\end{figure}

Hence, to sense differential phase from the sensor, the wireless reader reads the phases at shifted frequencies, and observes the phase jumps caused by the shifting of contact edges between the traces due to an applied force (Fig.~\ref{fig:contactlength}). 
Denote the reflected signal just before/after a contact force was applied as $r_1(t)/r_2(t)$. From, Fig.~\ref{fig:contactlength} $\angle r_1(t) = \phi_{\text{full}}+\phi_a$, from the wireless propagation over the air and over the entire length of the sensor. Similarly, $\angle r_2(t) = \phi_{\text{short}}+\phi_a$, since now the signal got reflected back from the shorting point. 
Thus, the differential phase between $r_1(t), r_2(t)$ would be $\phi_{\text{full}}+\cancel{\phi_{a}}-\phi_{\text{short}}-\cancel{\phi_a}$, and thus the differential phase jump would give us $\phi_{\text{full}}-\phi_{\text{short}}$. Since $\phi_{\text{full}}$ is the net phase accumulated by the signals by traveling the full length of the microstrip line, this is a fixed quantity that can be calibrated beforehand from accurate VNA readings. Thus, reading the differential phase allows us to estimate  $\phi_{\text{full}}-\phi_{\text{short}}$, and in turn, $\phi_{\text{short}}$, which is the phase due to the shifting of contact points caused by an applied force. 

% Why naiveity wont work
\noindent \textbf{Sensing differential phase from both the ends of the sensor:} A naive extension to the single ended measurement is to have RF switches on both ends of the sensor, toggle them at different frequencies ($f_{s_1}/f_{s_2}$), and read the phase jumps at these shifted frequencies. Although this solution to sense phase jumps from both ends is correct in spirit, there is more to the double-ended sensing problem than just simple frequency multiplexing. To estimate the differential phase, it is required to sense the phase before force was applied, in which the sensor acts like a perfectly conducting microstrip line between the two ends. In this scenario, if both the switches are toggled-on, the signals will propagate through the sensor and leak out from the other end. This causes intermodulated reflections, where the reflected signal would be partially modulated by both toggling frequencies. This is visually illustrated in Fig.~\ref{fig:intermod}.

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{figures/intermod.pdf}
\caption{Different freq. clocks introduce intermodulation due to both switches being toggled on (red shaded time instants)}
\label{fig:intermod}
\end{figure}
% Hence, the question to be posed is, how to avoid this intermodulation issue? When one switch is toggled-on to connect to the sensor, the other switch has to be toggled-off to act like an open reflector\footnote{The design setup hence requires reflective RF switches}, in order to avoid the intermodulation outputs.
The challenge in avoiding the intermodulation effects is that the sensor has to reflect signals from the opposite end when a switch is toggled on. Using reflective RF switches in the off state allows us to make either of the ends reflective, under the restriction that the other should be off when one switch is on.
\if 0
 By observing this, a naive attempt would be to consider time multiplexing instead. That is, at a given time only one switch toggles and the other is terminated, and after a definite time slot the roles reverse. However, this would then complicate the differential phase algorithm since it would be required to track the phase jumps arising due to clocks turning on and off. Further, it would limit the potential usage of multiple such sensors in tandem, since this time scheduling has to be agreed upon over multiple of these sensors. To bypass these issues, \paperTitle presents a unique clock design which would avoid the intermodulation issue and at the same time provide frequency separation for the reflected signals coming from either end.
\fi
The unique insight which allows \paperTitle to have such a on-off scheme is the use of duty cycle properties of square wave Fourier series. In a standard square wave, with $50\%$ duty cycle, all the even harmonics (i.e. every second harmonic) are absent. Similarly, in a wave with $25\%$ duty cycle, every fourth harmonic would be absent. Hence, a frequency $f_s$, $25\%$ duty cycle square wave will give modulation at $\underline{\mathbf{f_s}},2f_s,3f_s,\cancel{4f_s} 5f_s, \ldots$  Similarly, a frequency $2f_s$, $25\%$ duty cycle square wave will give modulation at $2f_s,\underline{\mathbf{4f_s}},6f_s,\cancel{8f_s},10f_s\ldots$ Observe that a combination of these 2 clocks will cause interference at $2f_s$, but can be read up individually at $f_s$ for the former clock, and $4f_s$ for the latter clock. Hence, a combination of these 2 clocks can provide separation in the frequency domain. Also, by controlling the initial phases of these two clocks, we can suppress the intermodulation problem as well. This is possible because when one clock is high, the other clock will be guaranteed to be low and vice versa (Fig.~\ref{fig:two-sided}). Hence, at any given time, only one port will be on, and other port will be reflective open. Further, to reduce the form factor requirements, instead of having $2$ antennas, one for each end of the sensor, we can just have just a one antenna design using a splitter. Since the clocking strategy provides separation in the frequency domain, we can add the modulated signals from the either ends via a splitter. Thus, we can read the differential phases at $f_s, 4f_s$ due to new shorting points caused by the bending of the sensor under an applied force $F$.
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{figures/twoended_design.pdf}
\caption{The two-ended sensing approach of \paperTitle. At any time instant, only one switch is toggled on}
\label{fig:two-sided}
\end{figure}

\subsection{Rejecting Multipath by Reading Forces at Multiple Frequencies}
\label{Subsec:wideband}

\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures/fft_ofdmalgo.pdf}
\caption{\paperTitle's sensing algorithm which utilizes wideband channel estimates to isolate the signal from multipath in Doppler domain. Finally, by grouping the channel estimates into `phasegroups', \paperTitle can read phase changes over multiple subcarriers which allows for averaging gains to make the phase sensing robust and accurate}
\label{fig:ofdm_expl}
\vspace{4mm}
\end{figure*}

% By utilizing the clock design strategy discussed, phases from both ends of the sensor are modulated with different shifted frequencies, which distinguish them from the excitation signal which is received directly without any frequency shifts. 
In this section, we describe how \name uses general wideband signals to measure differential phase across both ends of the sensor. The key insight of \paperTitle here is to use the general wide-band signal to estimate channel periodically and leverage these measurement to detect the frequency shifts coming from the sensor modulations. Further, going one step ahead, we can even harness tremendous averaging gains by reading the same differential phase over the entire wide-band channel estimates.
% In contrast, most of the past phase sensing solutions for RFID based touch sensing have largely used narrowband sensing, which further require a specialized RFID reader~\cite{pradhan2017rio}, whereas \paperTitle's solution can work with commodity 
% Thus, \paperTitle first comes up with a strategy to sense these phases from periodic channel estimates. 
Therefore, \name's strategy becomes waveform-agnostic, and can be used with any wideband sensing waveform that allows for periodic channel estimates, such as FMCW, UWB and WiFi-OFDM (11g).

\paperTitle's strategy consists of two steps: 
The first step involves viewing the frequency shift originating from square wave modulation as an `artificial-Doppler', since Doppler effects also introduce similar frequency shifts.
\name utilizes an FFT-based technique of sensing these frequency shifts, which works very similar to how Doppler is traditionally sensed via wideband sensing waveforms like FMCW and UWB~\cite{josephson2019rf}. We show that this algorithm works with a lower bandwidth (12.5 Mhz) OFDM based channel sounding approach. Since force information is in the form of phase changes unaffected by environmental effects and air propagation, we do not need absolute time-of-flight measurements, avoiding very high bandwidth (100s of MHz) typical of FMCW/UWB. 

\if 0
\notdone{\%\% The next few lines motivate the sensing strategy can be used in intro as well, just writing it here to put these thoughts into words \%\%}
Also, making the sensor design work with OFDM-based channel sounding provides interesting opportunities for communication and sensing to co-exist and allows for seamless future integration with Wi-Fi-based solutions. Further, in doing so we introduce a paradigm shift in backscatter sensing solutions, wherein, we don't require the quantization of data into bits and the sending of them over a low throughput link, but the data is instead embedded in the phase differences in channel estimates, and can be read continuously at the receiver. The former strategy requires presence of low power ADCs/data buffers to quantize and communicate the data, in addition to RF switches to isolate the reflected signal from excitation signal, whereas our solution just requires RF switches toggling with a certain clocking strategy. To justify the usage of these ADCs/data buffers, the former strategy requires presence of an explicit wake-up signal so that these power hungry components are used only for a fraction of time. In comparison, our design does not require the presence of such wake-up signals and can be turned-on all the time. Hence, we believe this sensing paradigm would pave the way forward to ultra low-power backscatter sensing links, which can work even in challenging environments like inside body tissue, where the efficiency of RF harvesters might not be able to support the sensing paradigms requiring ADCs/data buffers. \notdone{\%\% End of sensing motivation block\%\%}
\fi 
% Hence, now we will present how \paperTitle uses OFDM channel sounding to read the phase changes coming from either end of the sensor. 


The algorithm to estimate the two-ended differential phase embedded inside the wideband channel estimates is visually illustrated in Fig.~\ref{fig:ofdm_expl}. Say we are estimating the channel periodically after every $T$ seconds, with frequency steps of $F$ (this could be subcarrier spacing/sweep step in OFDM/FMCW based waveforms). We denote $H(kF,nT) = H[k,n]$ where $k$ is subcarrier index and $n$ is time index. Now, if there are $M$ multipaths in addition to the signal coming from the sensor, we can write the channel estimates as $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + (s_1(nT) e^{-j\phi^1_n} +s_2(nT)e^{-j\phi^2_n})\alpha_s e^{-j2\pi k F \frac{d_s}{c}}$

Here, $\alpha_i$ is the attenuation factor for the $i$-th path, $d_i$ is the distance separation between the TX-reflector and reflector-RX, and $\phi^1_n, \phi^2_n$ is the phase accumulated from the RF propagation in the microstrip line sensor at time index $n$ from sensor end $1$ and sensor end $2$. $s_1(t),s_2(t)$ are the double-ended sensor modulation as per the duty cycled clocking strategy discussed earlier. Expanding them as harmonics, we get $s_1(t) = \sum_{p\neq 4q, q\in \mathbb{Z}} a_p e^{j2\pi pf_{s_1}t}$, $s_2(t) = \sum_{p\neq 4q, q\in \mathbb{Z}} a_p e^{j2\pi pf_{s_2}t}$. We have $f_{s} = f_{s_1} = 0.5f_{s_2}$ and thus modulations at $f_{s}, 4f_{s}$. Ignoring the higher harmonics and the constant factors $a_p$ associated with the Fourier expansion for brevity, we get $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})$
% \begin{equation}
% \resizebox{0.45\textwidth}{!} 
% {
%     $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})$
% }
% \end{equation}
% \begin{equation}
% \begin{split}
%  H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} +&  \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+\\ &e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})
%  \end{split}
% \end{equation}

Now, to isolate the signal coming from the sensor, we take FFT over the $n$-th index, to obtain $\tilde{H}[k,f]$. We observe $N$ channel snapshots and take the following transform:
\begin{equation}
\tilde{H}[k,f] = \sum_{n=1}^N H[k,n] e^{-j2\pi f n T}
\end{equation}

Observe that for this transform, the nyquist frequency would be $\frac{1}{2T}$, and hence, $f_s$ has to be chosen such that $4f_s \leq \frac{1}{2T}$. Hence, assuming $\phi^1_n, \phi^2_n$ stay constant over the period of $N$ snapshots, at $f_s$, $4f_s$, we have,
\begin{equation}
\begin{split}
\tilde{H}[k,f_s] &= \sum_{n=1}^N H[k,n] e^{-j2\pi f_s n T} = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^1_n}\\
\tilde{H}[k,4f_s] &= \sum_{n=1}^N H[k,n] e^{-j2\pi 4f_s n T} = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^2_n}\\
\end{split}
\label{eqn:sensharmonics}
\end{equation}

This draws a parallel to how Doppler is sensed from wideband sensing algorithms, and switching in fact gives the sensor an `artificial Doppler' which can be sensed as done above. The switching frequency $f_s$ can be related to an equivalent Doppler, $f_s = \frac{f_c v}{c}$, and thus an object in the environment moving at velocity $v = \frac{c f_s}{f_c}$ would create interference with the sensor signal. However, the chosen $f_s$ is large enough so that this equivalent speed is so high that it wouldn't appear in the environment for the use cases considered. Hence, taking this FFT isolates the signal coming from the sensor and nulls out the multipath clutter in the environment. 

Recall that while writing Eqn.~\eqref{eqn:sensharmonics}, we assumed $\phi^1_n, \phi^2_n$ stay constant over the period of $N$ snapshots. Basically, this assumes that the force acting on the sensor stays almost constant for about $N$ snapshots, which is a reasonable assumption given it requires some time for mechanical beams to relax and get to steady state under the action of force. Said differently, wireless sensing occurs at much higher sampling rate (about order of MHz), whereas the mechanical forces are much slower (take about 0.5-1 seconds to stabilize). 

Thus, \paperTitle designs an algorithm to sense these phase differences from the filtered harmonics, and ultimately map them to applied force. The algorithm divides the channel estimates into groups of $N$, referred to as `phase-groups'. For each phase-group we first take the harmonics FFT as described earlier and obtain $2$ $K\times1$ vector from Eqn.\ref{eqn:sensharmonics} for FFT frequency $f_s$, $4f_s$. Assuming there are $N_g$ such phase groups, and for all $N$ samples of $g$-th group, $\phi^1_n,\phi^2_n \approx \phi^1_g \phi^2_g \forall n \in \{1,2,\ldots N\}$. The output at $g$-th phase group, $k$-th subcarrier, after harmonics FFT at $f_s, 4f_s$, is denoted as $P_1[k,g],P_2[k,g]$, and has the following form:
\begin{equation}
\begin{split}
P_1[k,g] &=\tilde{H}[k,f_s] = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^1_g}\\
P_2[k,g] &=\tilde{H}[k,4f_s] = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^2_g}
\end{split}
\end{equation}

Hence, we can obtain the phase change between 2 groups $\phi^1_{g+1}-\phi^1_{g}, \phi^2_{g+1}-\phi^2_{g}$ due to some contact force applied during this time by taking conjugate multiplication:
\begin{equation}
\begin{split}
\tilde{P}_1[k,g] &= P_1[k,g+1]*\text{conj}(P_1[k,g]) \\
           &= \alpha_s \cancel{e^{-j2\pi k F \frac{d_s}{c}}} e^{j\phi^1_{g+1}} \alpha^{*}_s \cancel{e^{j2\pi k F \frac{d_s}{c}}} e^{-j\phi^1_g+1}\\
           & = |\alpha_s|^2 e^{j(\phi^1_{g+1}-\phi^1_g)}
\end{split}
\end{equation}
Hence, we have
\begin{equation}
\angle{\tilde{P}_1[k,g]} = \phi^1_{g+1}-\phi^1_g, \angle{\tilde{P}_2[k,g]} = \phi^2_{g+1}-\phi^2_g 
\end{equation}
for each subcarrier $k$. We can assume that the required phase change is almost constant with subcarrier index given the low bandwidth, ($f_c+k\Delta F \sim f_c$). This allows us to measure the phase change at multiple subcarriers and finally we can take an average (over subcarrier indices $k$) here to get to one sample value of phase change from either sides of the sensor. Thus by observing $\text{mean}(\angle{\tilde{P}_1[k,g]}), \text{mean}(\angle{\tilde{P}_2[k,g]})$ over multiple phase groups, we can identify the action of a contact force $F$ which acts on the sensor and induces these phase changes.



==> wideband_sec_old.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures/fft_ofdmalgo.pdf}
\caption{\paperTitle's sensing algorithm which utilizes wideband channel estimates to isolate the signal from multipath in Doppler domain. Finally, by grouping the channel estimates into `phasegroups', \paperTitle can read phase changes over multiple subcarriers which allows for averaging gains to make the phase sensing robust and accurate}
\label{fig:ofdm_expl}
\vspace{4mm}
\end{figure*}

% By utilizing the clock design strategy discussed, phases from both ends of the sensor are modulated with different shifted frequencies, which distinguish them from the excitation signal which is received directly without any frequency shifts.
% \todo{\%\% Don't Review: to be re-written \% \%}
Till now, we have described the phase-force transduction mechanism, and delineated a method to give disambiguated identities to both ends of the sensor. Now, in this section, we move on to the description of how the wireless reader is designed. At the cornerstone of the design principle for our wireless reader, lies the fact that the force magnitude and location can be recovered by sensing `differential phase'.
Hence, we design our wireless reader to detect the separate identities stemming from frequency shifts, and then extract the valuable phase information which allows us to sense and localize forces.
% In this section, we describe how \name uses general wideband signals to measure differential phase across both ends of the sensor. 
The key insight of \paperTitle here is to use the general wide-band signal to estimate channel periodically and leverage these measurement to detect the frequency shifts coming from the sensor modulations. Further, going one step ahead, we can even harness tremendous averaging gains by reading the same differential phase over the entire wide-band channel estimates.
% In contrast, most of the past phase sensing solutions for RFID based touch sensing have largely used narrowband sensing, which further require a specialized RFID reader~\cite{pradhan2017rio}, whereas \paperTitle's solution can work with commodity 
% Thus, \paperTitle first comes up with a strategy to sense these phases from periodic channel estimates. 
% Therefore, \name's strategy becomes waveform-agnostic, and can be used with any wideband sensing waveform that allows for periodic channel estimates, such as FMCW, UWB and WiFi-OFDM (11g).

\paperTitle's strategy consists of two steps: 
The first step involves viewing the frequency shift originating from square wave modulation as an `artificial-Doppler', since Doppler effects also introduce similar frequency shifts.
\name utilizes an FFT-based technique of sensing these frequency shifts, which works very similar to how Doppler is traditionally sensed via wideband sensing waveforms like FMCW and UWB~\cite{josephson2019rf}. We show that this algorithm works with a lower bandwidth (12.5 Mhz) OFDM based channel sounding approach. Since force information is in the form of phase changes unaffected by environmental effects and air propagation, we do not need absolute time-of-flight measurements, avoiding very high bandwidth (100s of MHz) typical of FMCW/UWB. 

\if 0
\notdone{\%\% The next few lines motivate the sensing strategy can be used in intro as well, just writing it here to put these thoughts into words \%\%}
Also, making the sensor design work with OFDM-based channel sounding provides interesting opportunities for communication and sensing to co-exist and allows for seamless future integration with Wi-Fi-based solutions. Further, in doing so we introduce a paradigm shift in backscatter sensing solutions, wherein, we don't require the quantization of data into bits and the sending of them over a low throughput link, but the data is instead embedded in the phase differences in channel estimates, and can be read continuously at the receiver. The former strategy requires presence of low power ADCs/data buffers to quantize and communicate the data, in addition to RF switches to isolate the reflected signal from excitation signal, whereas our solution just requires RF switches toggling with a certain clocking strategy. To justify the usage of these ADCs/data buffers, the former strategy requires presence of an explicit wake-up signal so that these power hungry components are used only for a fraction of time. In comparison, our design does not require the presence of such wake-up signals and can be turned-on all the time. Hence, we believe this sensing paradigm would pave the way forward to ultra low-power backscatter sensing links, which can work even in challenging environments like inside body tissue, where the efficiency of RF harvesters might not be able to support the sensing paradigms requiring ADCs/data buffers. \notdone{\%\% End of sensing motivation block\%\%}
\fi 
% Hence, now we will present how \paperTitle uses OFDM channel sounding to read the phase changes coming from either end of the sensor. 


The algorithm to estimate the two-ended differential phase embedded inside the wideband channel estimates is visually illustrated in Fig.~\ref{fig:ofdm_expl}. Say we are estimating the channel periodically after every $T$ seconds, with frequency steps of $F$ (this could be subcarrier spacing/sweep step in OFDM/FMCW based waveforms). We denote $H(kF,nT) = H[k,n]$ where $k$ is subcarrier index and $n$ is time index. Now, if there are $M$ multipaths in addition to the signal coming from the sensor, we can write the channel estimates as $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + (s_1(nT) e^{-j\phi^1_n} +s_2(nT)e^{-j\phi^2_n})\alpha_s e^{-j2\pi k F \frac{d_s}{c}}$

Here, $\alpha_i$ is the attenuation factor for the $i$-th path, $d_i$ is the distance separation between the TX-reflector and reflector-RX, and $\phi^1_n, \phi^2_n$ is the phase accumulated from the RF propagation in the microstrip line sensor at time index $n$ from sensor end $1$ and sensor end $2$. $s_1(t),s_2(t)$ are the double-ended sensor modulation as per the duty cycled clocking strategy discussed earlier. Expanding them as harmonics, we get $s_1(t) = \sum_{p\neq 4q, q\in \mathbb{Z}} a_p e^{j2\pi pf_{s_1}t}$, $s_2(t) = \sum_{p\neq 4q, q\in \mathbb{Z}} a_p e^{j2\pi pf_{s_2}t}$. We have $f_{s} = f_{s_1} = 0.5f_{s_2}$ and thus modulations at $f_{s}, 4f_{s}$. Ignoring the higher harmonics and the constant factors $a_p$ associated with the Fourier expansion for brevity, we get $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})$
% \begin{equation}
% \resizebox{0.45\textwidth}{!} 
% {
%     $H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} + \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})$
% }
% \end{equation}
% \begin{equation}
% \begin{split}
%  H[k,n] = \sum_{i=1}^M \alpha_i e^{-j2\pi k F \frac{d_i}{c}} +&  \alpha_s e^{-j2\pi k F \frac{d_s}{c}}  (e^{j2\pi f_{s}nT}e^{-j\phi^1_n}+\\ &e^{j2\pi (4f_{s})nT}e^{-j\phi^2_n})
%  \end{split}
% \end{equation}

Now, to isolate the signal coming from the sensor, we take FFT over the $n$-th index, to obtain $\tilde{H}[k,f]$. We observe $N$ channel snapshots and take the following transform:
\begin{equation}
\tilde{H}[k,f] = \sum_{n=1}^N H[k,n] e^{-j2\pi f n T}
\end{equation}

Observe that for this transform, the nyquist frequency would be $\frac{1}{2T}$, and hence, $f_s$ has to be chosen such that $4f_s \leq \frac{1}{2T}$. Hence, assuming $\phi^1_n, \phi^2_n$ stay constant over the period of $N$ snapshots, at $f_s$, $4f_s$, we have,
\begin{equation}
\begin{split}
\tilde{H}[k,f_s] &= \sum_{n=1}^N H[k,n] e^{-j2\pi f_s n T} = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^1_n}\\
\tilde{H}[k,4f_s] &= \sum_{n=1}^N H[k,n] e^{-j2\pi 4f_s n T} = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^2_n}\\
\end{split}
\label{eqn:sensharmonics}
\end{equation}

This draws a parallel to how Doppler is sensed from wideband sensing algorithms, and switching in fact gives the sensor an `artificial Doppler' which can be sensed as done above. The switching frequency $f_s$ can be related to an equivalent Doppler, $f_s = \frac{f_c v}{c}$, and thus an object in the environment moving at velocity $v = \frac{c f_s}{f_c}$ would create interference with the sensor signal. However, the chosen $f_s$ is large enough so that this equivalent speed is so high that it wouldn't appear in the environment for the use cases considered. Hence, taking this FFT isolates the signal coming from the sensor and nulls out the multipath clutter in the environment. 

Recall that while writing Eqn.~\eqref{eqn:sensharmonics}, we assumed $\phi^1_n, \phi^2_n$ stay constant over the period of $N$ snapshots. Basically, this assumes that the force acting on the sensor stays almost constant for about $N$ snapshots, which is a reasonable assumption given it requires some time for mechanical beams to relax and get to steady state under the action of force. Said differently, wireless sensing occurs at much higher sampling rate (about order of MHz), whereas the mechanical forces are much slower (take about 0.5-1 seconds to stabilize). 

Thus, \paperTitle designs an algorithm to sense these phase differences from the filtered harmonics, and ultimately map them to applied force. The algorithm divides the channel estimates into groups of $N$, referred to as `phase-groups'. For each phase-group we first take the harmonics FFT as described earlier and obtain $2$ $K\times1$ vector from Eqn.\ref{eqn:sensharmonics} for FFT frequency $f_s$, $4f_s$. Assuming there are $N_g$ such phase groups, and for all $N$ samples of $g$-th group, $\phi^1_n,\phi^2_n \approx \phi^1_g \phi^2_g \forall n \in \{1,2,\ldots N\}$. The output at $g$-th phase group, $k$-th subcarrier, after harmonics FFT at $f_s, 4f_s$, is denoted as $P_1[k,g],P_2[k,g]$, and has the following form:
\begin{equation}
\begin{split}
P_1[k,g] &=\tilde{H}[k,f_s] = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^1_g}\\
P_2[k,g] &=\tilde{H}[k,4f_s] = \alpha_s e^{-j2\pi k F \frac{d_s}{c}} e^{j\phi^2_g}
\end{split}
\end{equation}

Hence, we can obtain the phase change between 2 groups $\phi^1_{g+1}-\phi^1_{g}, \phi^2_{g+1}-\phi^2_{g}$ due to some contact force applied during this time by taking conjugate multiplication:
\begin{equation}
\begin{split}
\tilde{P}_1[k,g] &= P_1[k,g+1]*\text{conj}(P_1[k,g]) \\
           &= \alpha_s \cancel{e^{-j2\pi k F \frac{d_s}{c}}} e^{j\phi^1_{g+1}} \alpha^{*}_s \cancel{e^{j2\pi k F \frac{d_s}{c}}} e^{-j\phi^1_g+1}\\
           & = |\alpha_s|^2 e^{j(\phi^1_{g+1}-\phi^1_g)}
\end{split}
\end{equation}
Hence, we have
\begin{equation}
\angle{\tilde{P}_1[k,g]} = \phi^1_{g+1}-\phi^1_g, \angle{\tilde{P}_2[k,g]} = \phi^2_{g+1}-\phi^2_g 
\end{equation}
for each subcarrier $k$. We can assume that the required phase change is almost constant with subcarrier index given the low bandwidth, ($f_c+k\Delta F \sim f_c$). This allows us to measure the phase change at multiple subcarriers and finally we can take an average (over subcarrier indices $k$) here to get to one sample value of phase change from either sides of the sensor. Thus by observing $\text{mean}(\angle{\tilde{P}_1[k,g]}), \text{mean}(\angle{\tilde{P}_2[k,g]})$ over multiple phase groups, we can identify the action of a contact force $F$ which acts on the sensor and induces these phase changes.
